Improving Cooperative Adaptive Cruise Control Robustness to Parametric Uncertainty via Plant Equivalent Controller Realizations

Cooperative Adaptive Cruise Control (CACC) enables vehicle platooning through inter-vehicle communication, improving traffic efficiency and safety. Conventional CACC relies on feedback linearization, assuming exact knowledge of vehicle parameters. However, the nonlinear longitudinal vehicle dynamics are subject to parametric uncertainty. Applying such feedback linearization with a nominal model yields imperfect cancellation, leading to model mismatch and degraded performance with off-the-shelf CACC controllers. To improve robustness without redesigning the CACC law, we explicitly model the mismatch between the ideal closed-loop dynamics, assumed by the CACC design, and the actual dynamics under parametric uncertainties. Robustness is formulated as an $\mathcal{L}_2$ trajectory-matching problem, minimizing the energy of this mismatch to make the uncertain system behave as closely as possible to the ideal model. This objective is addressed by optimizing over plant equivalent controller (PEC) realizations that preserve the nominal closed-loop behavior while mitigating the effects of parametric uncertainty. Stability and performance are enforced via LMIs, yielding a convex optimization problem applicable to heterogeneous platoons. Experimental results demonstrate improved robustness and performance under parametric uncertainty while preserving nominal behavior.

==> 0.Bibligraphy.tex <==
\bibitem{guanetti_control_2018}
J. Guanetti, Y. Kim, and F. Borrelli, ``Control of connected and automated vehicles: {State} of the art and future challenges,'' \textit{Annual Reviews in Control}, vol. 45, 2018.

\bibitem{ghasemi_stable_2013}
A. Ghasemi, R. Kazemi, and S. Azadi, ``Stable {Decentralized} {Control} of a {Platoon} of {Vehicles} {With} {Heterogeneous} {Information} {Feedback},'' \textit{IEEE Trans. on Vehicular Tech.}, vol. 62, 2013.

\bibitem{ploeg_design_2011}
J. Ploeg, B. T. M. Scheepers, E. Van Nunen, N. Van De Wouw, and H. Nijmeijer, ``Design and experimental evaluation of cooperative adaptive cruise control,'' in \textit{{Conf.} on {Intel.} {Transp.} {Systems}}, 2011.

\bibitem{lefeber_cooperative_2020}
E. Lefeber, J. Ploeg, and H. Nijmeijer, ``{CACC} of {Heterogeneous} {Vehicle} {Platoons},'' \textit{IFAC-PapersOnLine}, vol. 53, 2020.

\bibitem{de_haan_cooperative_2025}
R. De Haan, T. P. J. Van Der Sande, E. Lefeber, and I. J. M. Besselink, ``Cooperative {Adaptive} {Cruise} {Control} for {Heterogeneous} {Platoons} {With} {Delays}: {Controller} {Design} and {Experiments},'' \textit{IEEE Trans. on Control Systems Tech.}, vol. 33, 2025.

\bibitem{wijnbergen_existence_2020}
P. Wijnbergen and B. Besselink, ``Existence of decentralized controllers for vehicle platoons: {On} the role of spacing policies and available measurements,'' \textit{Systems \& Control Letters}, vol. 145, 2020.

\bibitem{baldi_establishing_2021}
S. Baldi, D. Liu, V. Jain, and W. Yu, ``Establishing {Platoons} of {Bidirectional} {Cooperative} {Vehicles} {With} {Engine} {Limits} and {Uncertain} {Dynamics},'' \textit{IEEE Trans. on Intel. Transp. Systems}, vol. 22, 2021.

\bibitem{gao_robust_2016}
F. Gao, S. E. Li, Y. Zheng, and D. Kum, ``Robust control of heterogeneous vehicular platoon with uncertain dynamics and communication delay,'' \textit{IET Intel. Transport Systems}, vol. 10,  2016.

\bibitem{li_robust_2018}
S. E. Li, F. Gao, K. Li, L. Wang, K. You, and D. Cao, ``Robust {Longitudinal} {Control} of {Multi}-{Vehicle} {Systems}—{A} {Distributed} {H}-{Infinity} {Method},'' \textit{IEEE Trans. on Intel. Transp. Systems}, vol. 19, 2018.

\bibitem{zhu_adaptive_2019}
Y. Zhu, D. Zhao, and Z. Zhong, ``Adaptive {Optimal} {Control} of {Heterogeneous} {CACC} {System} {With} {Uncertain} {Dynamics},'' \textit{IEEE Trans. on Control Systems Tech.}, vol. 27, 2019.

\bibitem{quan_robust_2024}
Y. S. Quan, J. S. Kim, and C. C. Chung, ``Robust {Adaptive} {Cruise} {Control} {Design} {Using} {MPC},'' \textit{IEEE Trans. on Intel. Vehicles}, 2024.

\bibitem{yang_adaptive_2023}
X. Yang, E. Lefeber, C. Wu, H. Yi, and Z. Zheng, ``Adaptive {Controller} {Design} for {Heterogeneous} {CACC} {System} with {Uncertain} {Vehicle} {Parameters},'' \textit{Int. Conf. on Intel.
Transp. Systems}, 2023.

\bibitem{xing_robust_2022}
H. Xing, J. Ploeg, and H. Nijmeijer, ``Robust {CACC} in the {Presence} of {Uncertain} {Delays},'' \textit{IEEE Trans. on Vehicular Tech.}, vol. 71, 2022.

\bibitem{alam_guaranteeing_2014}
A. Alam, A. Gattami, K. H. Johansson, and C. J. Tomlin, ``Guaranteeing safety for heavy duty vehicle platooning: {Safe} set computations and experimental evaluations,'' \textit{Control Engineering Practice}, 2014.

\bibitem{sheikholeslam_longitudinal_1993}
S. Sheikholeslam and C. A. Desoer, ``Longitudinal control of a platoon of vehicles with no communication of lead vehicle information: a system level study,'' \textit{IEEE Trans. on Vehicular Tech.}, vol. 42, 1993.

\bibitem{sahlholm_road_2010}
P. Sahlholm and K. H. Johansson, ``Road grade estimation for look-ahead vehicle control using multiple measurement runs,'' \textit{Control Engineering Practice}, vol. 18, 2010.

\bibitem{besselink_cyberphysical_2016}
B. Besselink, V. Turri, S. H. Van De Hoef, K. Liang, A. Alam, J. Martensson, and K. H. Johansson, ``Cyber–{Physical} {Control} of {Road} {Freight} {Transport},'' \textit{Proc. of the IEEE}, vol. 104, 2016.

\bibitem{huisman_optimal_2024}
M. Huisman, C. Murguia, E. Lefeber, and N. Van De Wouw, ``Optimal {Controller} {Realizations} against {False} {Data} {Injections} in {Cooperative} {Driving},'' in \textit{Proc. IEEE CDC}, 2024.

\bibitem{huisman_plant_2025}
M. Huisman, E. Lefeber, N. van de Wouw, and C. Murguia, ``Plant {Equivalent} {Controller} {Realizations} for {Attack}-{Resilient} {Cyber}-{Physical} {Systems},'' 2025. [Online]. Available: https://arxiv.org/abs/2512.13229.

\bibitem{ding_model-based_2013}
S. X. Ding, \textit{Model-{Based} {Fault} {Diagnosis} {Techniques}: {Design} {Schemes}, {Algorithms} and {Tools}}, Springer London, 2013.

\bibitem{boyd_linear_1994}
S. P. Boyd (Ed.), \textit{Linear matrix inequalities in system and control theory}, Society for Industrial and Applied Mathematics, 1994.

\bibitem{Lofberg2004}
J. Lofberg, ``{YALMIP}: Toolbox for Modeling and Optimization,'' 2004.

\bibitem{mosek}
{MOSEK ApS}, \textit{The {MOSEK} optimization toolbox for {MATLAB}.}, 2024. 


==> 1.Introduction_V1.tex <==
\section{INTRODUCTION} \vspace{-1mm}
Cooperative Adaptive Cruise Control (CACC) is a well-explored technology for improving traffic throughput, fuel efficiency, and safety in intelligent transportation systems. Enabling CACC through Vehicle-to-Vehicle communication allows vehicles to form platoons and closely follow one another while maintaining string stability~\cite{guanetti_control_2018}.

Many CACC designs, as well as other longitudinal controllers, rely on an additional nonlinear control layer that performs feedback linearization of the vehicle dynamics to facilitate controller design and analysis~\cite{ghasemi_stable_2013, ploeg_design_2011, lefeber_cooperative_2020, de_haan_cooperative_2025, wijnbergen_existence_2020}. However, feedback linearization inherently assumes exact knowledge of vehicle and road parameters, such as mass, aerodynamic drag, viscous friction, and driveline dynamics. In practice, these parameters are uncertain and may vary significantly over time, for instance, due to changing payload conditions in heavy-duty vehicles, which can lead to instability and performance degradation if not accounted for.

To address model uncertainty in platoons, a variety of robust and adaptive control strategies have been proposed in the literature. Extensive research has focused on uncertainty in driveline dynamics, including online driveline parameter estimation~\cite{baldi_establishing_2021}, robust $\mathcal{H}_\infty$ control methods~\cite{gao_robust_2016,li_robust_2018}, and self-learning techniques~\cite{zhu_adaptive_2019}. Other approaches consider additional sources of uncertainty, such as wind gusts, which are addressed using robust model predictive control in~\cite{quan_robust_2024}. Nonlinear adaptive CACC schemes with online parameter updates have also been investigated~\cite{yang_adaptive_2023}, although such methods may be sensitive to measurement noise. Furthermore, adaptive control strategies that account for uncertain communication and actuation delays are proposed in \cite{xing_robust_2022, de_haan_cooperative_2025}.

Despite these advances, the existing approaches typically focus on specific subsets of uncertainty or rely on simplified vehicle models, even though nonlinear dynamics and their uncertainties play an important role in, e.g., safety-critical scenarios~\cite{alam_guaranteeing_2014}. Therefore, this paper first introduces a general nonlinear longitudinal vehicle model that explicitly accounts for multiple resistive forces, following established modeling approaches \cite{sheikholeslam_longitudinal_1993, sahlholm_road_2010, alam_guaranteeing_2014, besselink_cyberphysical_2016}. Feedback linearization is then applied without assuming exact knowledge of all model parameters, allowing uncertainty not only in driveline dynamics or wind velocity, but also in vehicle mass, effective mass, and aerodynamic drag and viscous friction coefficients.

To enhance the robustness and performance of the closed-loop system in the presence of parametric model uncertainty, we exploit plant equivalent (PEC) realizations~\cite{huisman_optimal_2024,huisman_plant_2025}. We leverage degrees of freedom in the realization of a given dynamic CACC scheme, referred to herein as the \emph{base controller}, to mitigate the impact of uncertainty without altering the desired nominal performance. By appropriately selecting the PEC realization, the propagation of parametric uncertainty through the closed-loop dynamics can be mitigated. By defining nominal and uncertainty-induced error states, the proposed framework enables systematic tuning of the controller realization to minimize both transient and steady-state performance degradation, while guaranteeing stability.

The resulting closed-loop system is formulated as a polytopic uncertain linear system, where the PEC realization design variables enter linearly. This structure allows robust stability and performance to be enforced through a set of linear matrix inequalities evaluated at the vertices of the uncertainty polytope. The design objective combines the minimization of the average output energy induced by uncertainty with bounds on the worst-case input-output gain (i.e., $\mathcal{H}_\infty$), yielding a convex optimization problem that can be efficiently solved using SDP solvers. The proposed PEC realizations apply to heterogeneous platoons, while explicitly optimizing performance with respect to model uncertainty. The proposed method is experimentally validated on a vehicle, demonstrating improved robustness under uncertainty.

The remainder of this paper is organized as follows. Section~\ref{sec:Preliminaries} introduces the required preliminaries. Section~\ref{sec:ProblemSetting} presents the nonlinear vehicle model and introduces the PEC realizations. Section~\ref{sec:approach} describes the framework for robust stability and performance optimization using PEC realizations. Section~\ref{sec:Results} compares simulation and experimental results, and Section~\ref{sec:Conclusion} concludes the paper.

==> 2_Preliminaries/2.2_Definition_V1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Definitions} 

\begin{definition}[Polytopic uncertain system \cite{ding_model-based_2013,boyd_linear_1994}] \
\label{def:polytopic_system}
Consider the linear system with model uncertainties
\begin{subequations}\begin{align}
    \dot{x}(t) &= A(\Delta) x(t) + B(\Delta) u(t), \\
    y(t) &= C(\Delta) x(t) + D(\Delta) u(t),
\end{align}\end{subequations}
where $x(t) \in \mathbb{R}^n$ is the state, $u(t) \in \mathbb{R}^m$ is the input, $y(t) \in \mathbb{R}^r$ is the output. For a polytopic uncertain system, matrices $A(\Delta),\, B(\Delta),\, C(\Delta),$ and $D(\Delta)$ are subject to parametric uncertainty and belong to a convex polytope $\Omega := \mathrm{conv}\left\{ S^{[1]}, S^{[2]}, \dots, S^{[N]} \right\}$, where each vertex $S^{[k]}$ is defined as a tuple
\begin{align}
    S^{[k]} := \left( A^{[k]}, B^{[k]}, C^{[k]}, D^{[k]} \right), \quad k = 1,\dots,N.
\end{align}
Accordingly, for any admissible uncertainty $\Delta$, the system matrices admit the representation
\begin{align}
    \Omega = \sum_{k=1}^{N} \alpha_k S^{[k]}, \, \sum_{k=1}^{N} \alpha_k = 1, \, \alpha_k \geq 0, \, k = 1,\dots,N.
\end{align}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Quadratic Stability~\cite{ding_model-based_2013,boyd_linear_1994}] \
\label{lemma1}
Consider the polytopic system described in Definition~\ref{def:polytopic_system} with $u(t) = 0$. If there exists a matrix $P \in \mathbb{R}^{n \times n}$ such that $P \succ 0$ and
\begin{align}
    ({A}^{[k]})^\top P + P {A}^{[k]} \prec 0, \quad \forall k \in \{1, \dots, N\},
\end{align}
then the origin of the system is asymptotically stable for all admissible uncertainties $\Delta$.
\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Bounded Real Lemma~\cite{ding_model-based_2013,boyd_linear_1994}] \
\label{lemma2}
Consider the polytopic system in Definition~\ref{def:polytopic_system} with performance output
$z(t) = C_z(\Delta) x(t)$. If there exists a symmetric matrix $P \succ 0$ and a scalar $\gamma > 0$ such that, for all vertices $k = 1,\dots,N$,
\begin{align}
    \begin{bmatrix}
        (A^{[k]})^\top P + P A^{[k]} + (C_z^{[k]})^\top C_z^{[k]} & P B^{[k]} \\
        (B^{[k]})^\top P & -\gamma I
    \end{bmatrix} \preceq 0,
\end{align}
then the $\mathcal{L}_2$-gain from $u$ to $z$ satisfies $\| z \|_{\mathcal{L}_2} \leq \sqrt{\gamma} \| u \|_{\mathcal{L}_2}$,
for all admissible uncertainties $\Delta$ and all $u \in \mathcal{L}_2$.
\end{lemma}




==> 3_ProblemSetting/3.1_ProblemSetting_V1.tex <==
Consider a platoon of $m$ vehicles, schematically depicted in Fig. \ref{fig:SF_PlatoonModel}, where the vehicles are enumerated with index $i=1,...,m,$ with $i=1$ indicating the lead vehicle. Such a platoon is usually modeled using the longitudinal vehicle model \cite{ploeg_design_2011, lefeber_cooperative_2020}:
\begin{align} \label{eq:BG_PlatoonDynamics}
    \begin{bmatrix}
        \dot{d}_i \\ \dot{v}_i \\\dot{a}_i
    \end{bmatrix}
    = 
    \begin{bmatrix}
        \vim - v_i \\ a_i \\ -\frac{1}{\tau_i}a_i + \frac{1}{\tau_i} u_i
    \end{bmatrix}, \, i \in S_m \backslash \{1\},
\end{align}
where $d_i = q_{i-1} - q_i - L_i$ is the distance between vehicle $i$ and its preceding vehicle $i-1$, with $q_i$ denoting the position of the vehicle's rear bumper, and $L_i$ its length. Furthermore, $v_i$ and $a_i$ denote the velocity and acceleration of vehicle $i$, respectively, and $S_m \coloneqq \{ i \in \mathbb{N} \mid 1 \leq i \leq m \}$ (i.e., the set of all vehicles in a platoon of length $m \in \mathbb{N}$). The desired acceleration $u_i$ represents the control input of vehicle $i$, and $\tau_i>0$ is a time constant modeling driveline dynamics.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.8\linewidth]{00_Figures/PlatoonReduced.eps}
    \caption{CACC-equipped string of vehicles.}
    \label{fig:SF_PlatoonModel}
\end{figure}

The control objective for each follower vehicle is to keep a desired inter-vehicle distance $d_{r,i} = r_i + h_i v_i, \, i \in S_m \backslash \{ 1 \}$, with time gap $h_i>0$, and standstill distance $r_i>0$. The spacing error is defined as $e_i \coloneqq d_i - d_{r,i}$. To ensure this desired spacing and achieve string-stable vehicle-following behavior, a CACC scheme is introduced for a homogeneous platoon (i.e., $\tau_i = \tau\imo$) in~\cite{ploeg_design_2011}. However, in this work, we consider a heterogeneous platoon (i.e., $\tau_i \neq \tau\imo$). As discussed in~\cite{lefeber_cooperative_2020}, the CACC scheme from~\cite{ploeg_design_2011} in a heterogeneous platoon yields:
\begin{align} 
\label{eq:SD_BaseController} \vspace{-2mm} 
        \mathcal{F} &\coloneqq \left\{
        \begin{aligned}\begin{split}\dot{\rho}_i &= -\tfrac{1}{h} \rho_i + \tfrac{k_p}{h_i}e_i + \tfrac{k_d}{h_i} \dot{e}_i \\ & \qquad + \tfrac{\tau\imo - \tau_i}{h_i \tau\imo}\aim + \tfrac{\tau_i}{h_i \tau\imo}\uim, \end{split}\\
        u_i &= \rho_i, \end{aligned} \right.          
\end{align}
where $k_p>0$ and $k_d>0$ are control gains to be designed.

The model in \eqref{eq:BG_PlatoonDynamics} is obtained by applying input-output linearization to a nonlinear longitudinal vehicle model \cite{sheikholeslam_longitudinal_1993,sahlholm_road_2010, alam_guaranteeing_2014,besselink_cyberphysical_2016}. Such an input-output linearization relies on system parameters that are assumed to be known a priori. However, knowing all model parameters exactly is a strong assumption, since these quantities are typically known only approximately and may change over time, even for the same car. As a result, the desired closed-loop performance~\eqref {eq:BG_PlatoonDynamics}-~\eqref{eq:SD_BaseController} differs from the originally designed one.

To investigate the influence of these parameter uncertainties, we first define the nonlinear longitudinal dynamics of the $i$th vehicle. Then we perform the input-output linearization; however, rather than assuming perfect knowledge of the model, we incorporate model uncertainties $\Delta$. As a result, we have the desired linear model~\eqref{eq:BG_PlatoonDynamics}, but including a nonlinear function that maps the uncertainties onto the dynamics. For this uncertain system, the desired behavior of CACC controllers, as in~\cite{ploeg_design_2011,lefeber_cooperative_2020}, is not achieved. 

To enhance the robustness of the CACC scheme in~\eqref{eq:ploegHetero} against the model mismatch, we propose plant equivalent controller (PEC) realizations, i.e., distinct controller realizations producing the same control input~$u_i$ when $\Delta = 0$ while changing the internal dynamics on the dynamic controller. By defining a new controller state $\bar{\rho}_i$ via the linear change of coordinates \cite{huisman_optimal_2024, huisman_plant_2025}: 
\begin{align} \label{eq:PEC_Transformation}
  \bar{\rho}_i &=  \rho_i + \underbrace{\begin{bmatrix} f_{i,1} & f_{i,2} & f_{i,3} \end{bmatrix}}_{F_{1:3}} x_i + \underbrace{\begin{bmatrix} f_{i,4} & f_{i,5} \end{bmatrix}}_{F_{4:5}} x\imo.
\end{align} 
with $x_i = [d_i\, v_i\, a_i]^\top$ and $x\imo =[\vim \, \aim]^\top$ denoting the follower and leader states, respectively. This transformation yields a class of equivalent controller realizations that produce the same control input $u_i$ while depending on distinct sensor subsets. Applying~\eqref{eq:PEC_Transformation} to~\eqref{eq:SD_BaseController} yields:
\begin{subequations}\label{eq:rhoBar} \vspace{0mm}  \begin{align} 
    u_i &= \bar\rho_i - F_i x_i - F\imo x\imo, \\  
    \begin{split}
        \dot{\bar{\rho}}_i &= \left(\frac{f_{3}}{\tau_i}-\frac{1}{h}\right)\bar\rho_i + \begin{bmatrix} \bar b_{i,1} & \bar b_{i,2} & \bar b_{i,3}\end{bmatrix}  x_i \\
        & \qquad + \begin{bmatrix}\bar b_{i,4} & \bar b_{i,5}\end{bmatrix}  x\imo + b_{i,6} \uim,
    \end{split} \\
     \bar b_{i,1} &= \frac{k_p + f_{1}}{h_i} - \frac{f_{1}f_{3}}{\tau_i},\\ %% d2
     \bar b_{i,2} &= \frac{f_{2} - k_d}{h} - k_p - f_{1} - \frac{f_{2}f_{3}}{\tau_{i}},\\  %% v2 
     \bar b_{i,3} &= f_{2} - k_d + \frac{f_{3}}{h_i} - \frac{f_{3}(f_{3} + 1)}{\tau_{i}},\\ %% a2
     \bar b_{i,4} &= \frac{(f_{4} + k_d)}{h_i} + \frac{(f_{1}\tau_{i} - f_{3} f_{4})}{\tau_{i}},\\ %% v1
     \bar b_{i,5} &= \frac{f_{4} \tau_{i} - f_{3} f_{5}}{\tau_{i}} + \frac{f_{5} + 1}{h_i} - \frac{\tau_{i} + f_{5} h}{h \tau\imo},\\ %% a1
     \bar b_{i,6} &= \frac{(\tau_{i} + f_{5} h_i)}{h_i \tau\imo}, %% u1
 \end{align} \end{subequations} \vspace{0mm} 
where each pair ($\beta_{i,j},\bar{B}_{i,j}$) yields another controller realization, which in itself can depend on a different subset of sensors.

To this end, we exploit the concept of plant equivalent controller (PEC) realizations, which exhibit identical closed-loop performance when $\Delta = 0$. However, their response in case of uncertanties differ. We obtain an optimal controller realization by minimizing the error between the desired model using the bounded-real lemma. 













==> 3_ProblemSetting/3.1_ProblemSetting_V2.tex <==
Consider a platoon of $m$ vehicles, schematically depicted in Fig. \ref{fig:SF_PlatoonModel}, indexed by $i\in\,S_m \coloneqq \{1,\ldots,m\}$, where $i=1$ denotes the lead vehicle. The longitudinal dynamics of the $i$th vehicle are commonly modeled as~\cite{sheikholeslam_longitudinal_1993,sahlholm_road_2010,alam_guaranteeing_2014,besselink_cyberphysical_2016}
\begin{subequations}\label{eq:PF_NLModel}\begin{align}
    \dot{F}_{\text{drive},i} &= -\frac{F_{\text{drive},i}}{\tau_i} + \frac{\eta_i}{\tau_i}, \label{eq:PF_engDyn} \\
     m_{\text{eff},i} a_i &= F_{\text{drive},i} - F_{\text{d},i} - F_{\text{v},i} - F_{\text{r},i} - F_{g,i}, \label{eq:PF_accDyn}
\end{align}
where $m_{\text{eff},i}$ denotes the effective vehicle mass, $\tau_i$ the driveline time constant, $F_{\text{drive},i}$ the driving force, $\eta_i$ the engine input, and $a_i$ the acceleration of vehicle $i$. The resistive forces consist of aerodynamic drag $F_{\text{d},i}$, viscous friction $F_{\text{v},i}$, rolling resistance $F_{\text{r},i}$, and the gravitational component $F_{g,i}$ of vehicle $i$, which are defined as
\begin{align}   
    F_{\text{d},i} &= C_{\text{d},i} (v_i-v_\text{w} )^2, \qquad
    &&F_{\text{v},i} = f_{\text{v},i} v_i, \label{eq:PF_Forces} \\ 
    F_{\text{r},i} &\approx f_{\text{r},i} m_i g,  \,\,
    && F_{g,i} \approx m_i g \alpha_i,
\end{align}\end{subequations}
with $v_i$ the vehicle velocity, $C_{\text{d},i}$ the drag coefficient, $v_\text{w}$ the wind speed, $f_{\text{v},i}$ the viscous friction coefficient, $f_{\text{r},i}$ the rolling resistance coefficient, $m_i$ the vehicle mass, $g$ the gravitational constant, and $\alpha_i$ the road slope.

Assuming small road slopes $\alpha_i$, and slowly varying rolling and gravitational forces, differentiation of~\eqref{eq:PF_accDyn} together with~\eqref{eq:PF_Forces} yields the nonlinear acceleration dynamics
\begin{multline} \label{eq:PF_nlPlatoon}
     \hspace{-3.5mm}\dot{a}_i = - \tfrac{f_{\text{v},i} - 2C_{\text{d},i} v_\text{w}}{\tau_i m_{\text{eff},i}} v_i - \left(\tfrac{f_{\text{v},i} - 2C_{\text{d},i} v_\text{w}}{m_{\text{eff},i}} + \tfrac{1}{\tau_i} \right)a_i -\tfrac{C_{\text{d},i}}{\tau_i m_{\text{eff},i}}v_i^2 \\
    - \tfrac{2 C_{\text{d},i}}{m_{\text{eff},i}}v_i a_i - \tfrac{m_i(f_{\text{r},i} g + g \alpha_i) + C_{\text{d},i} v_\text{w}^2}{\tau_i m_{\text{eff},i}} + \tfrac{1}{\tau_i m_{\text{eff},i}} \eta_i.
\end{multline}
\begin{figure}[bt]
    \centering
    \includegraphics[width=\linewidth]{00_Figures/Platoon_nominal.eps}
    \caption{CACC-equipped string of vehicles.}
    \label{fig:SF_PlatoonModel}
    \vspace{-5mm}
\end{figure}

The control objective for each follower vehicle is to keep a desired inter-vehicle distance $d_{\text{r},i} = r_i + h_i v_i, \, i \in S_m \backslash \{ 1 \}$, with time gap $h_i>0$ and standstill distance $r_i\geq0$. Several CACC schemes have been proposed in the literature to achieve this objective, e.g.,~\cite{ploeg_design_2011,lefeber_cooperative_2020, de_haan_cooperative_2025}, which are based on a vehicle model obtained via feedback linearization of~\eqref{eq:PF_nlPlatoon}.

Feedback linearization is achieved via engine input $\eta_i$, and requires exact knowledge of all parameters in~\eqref{eq:PF_nlPlatoon}. Since this assumption is generally unrealistic, we introduce six parameter groups $p_j$, $j \in \{1,\ldots,6\}$, each characterized by a nominal estimate $p_{j|0}$ and an additive uncertainty $\Delta_j$. This allows rewriting~\eqref{eq:PF_nlPlatoon} as
\begin{multline}\label{eq:PF_nl_Uncertain}
   \! \! \! \dot{a}_i =  -(p_{1|0} + \Delta_1)v_i 
    - (p_{2|0} + \Delta_2)a_i 
    - (p_{3|0} + \Delta_{3})v_i^2 \\ 
    - (p_{4|0} + \Delta_{4}) v_i a_i 
    - (p_{5|0} + \Delta_5) 
    + (p_{6|0} + \Delta_6) \eta_i.
\end{multline}


Following~\cite{ploeg_design_2011,lefeber_cooperative_2020}, the desired vehicle model is defined as
\begin{subequations} \label{eq:desiredModel} \begin{align}
    \dot{q}_i &= v_i, \qquad \dot{v}_i = a_i, \\
    \dot{a}_i &= -\tfrac{1}{\tau_{\text{des},i}} a_i + \tfrac{1}{\tau_{\text{des},i}} u_i,  \label{eq:desiredModel_da} 
\end{align}\end{subequations}
with position $q_i$, velocity $v_i$, new input $u_i$ and design parameter $\tau_{\text{des},i} > 0$. Using the nominal parameter estimates $p_{j|0}$, the feedback linearizing control law yields
\begin{multline} \label{eq:PF_IOcontroller_param}
    \eta_i = p_{6|0}^{-1} \Big(
        p_{1|0} v_i
        + \Big(p_{2|0} - \tfrac{1}{\tau_{\text{des},i}}\Big) a_i
        + p_{3|0} v_i^2  \\
        + p_{4|0} v_i a_i
        + p_{5|0}
        + \tfrac{1}{\tau_{\text{des},i}} u_i
    \Big).
\end{multline}

Substituting~\eqref{eq:PF_IOcontroller_param} into~\eqref{eq:PF_nl_Uncertain} yields the perturbed dynamics
\begin{subequations}\label{eq:PF_simplified_uncertain}
\begin{align}
    \dot{a}_i &= - \tfrac{1}{\tau_{\text{des},i}} a_i
    + \tfrac{1}{\tau_{\text{des},i}} u_i
    + \phi_i, \\
    \begin{split}
    \phi_i
    &= \theta_{i,1} v_i
    + \theta_{i,2} a_i 
    + \theta_{i,3} v_i^2 
    + \theta_{i,4} v_i a_i \\
    & \qquad + \theta_{i,5} 
    + \theta_{i,6} u_i,
    \end{split}
\end{align}
with
\begin{align}\label{eq:theta1}
    \theta_{i,1} &= \tfrac{p_{1|0}}{p_{6|0}}\Delta_6 - \Delta_1, \\
    \theta_{i,2} &= \left(\tfrac{p_{2|0}}{p_{6|0}} - \tfrac{1} {p_{6|0}\tau_{\text{des},i}} \right) \Delta_6 - \Delta_2, \\
    \theta_{i,3} &= \tfrac{p_{3|0}}{p_{6|0}}\Delta_6 - \Delta_3, \qquad
    \theta_{i,4} = \tfrac{p_{4|0}}{p_{6|0}} \Delta_6 - \Delta_4, \\
    \theta_{i,5} &= \tfrac{p_{5|0}}{p_{6|0}} \Delta_6 - \Delta_5, \qquad 
    \theta_{i,6} = \tfrac{1}{p_{6|0}\tau_{\text{des},i}} \Delta_6. \label{eq:theta6}
\end{align}
\end{subequations}
In the absence of uncertainty (i.e., $\Delta = 0$),~\eqref{eq:PF_simplified_uncertain} reduces to the desired model~\eqref{eq:desiredModel}.

Consider the CACC scheme for a heterogeneous platoon (i.e., $\tau_{\text{des},i} \coloneqq \tau_i \neq \tau\imo$)~\cite{ploeg_design_2011,lefeber_cooperative_2020}:
\begin{align} 
    \label{eq:SD_BaseController} \vspace{-2mm} 
    \mathcal{F} &\coloneqq \left\{
    \begin{aligned}
        \begin{split}\dot{\rho}_i &= -\tfrac{1}{h} \rho_i + \tfrac{k_p}{h_i}e_i + \tfrac{k_d}{h_i} \dot{e}_i \\ & \qquad + \tfrac{\tau\imo - \tau_i}{h_i \tau\imo}\aim + \tfrac{\tau_i}{h_i \tau\imo}\uim, \end{split} \\ 
        u_i &= \rho_i, 
    \end{aligned} \right.          
\end{align}
where $e_i \coloneqq d_i - d_{\text{r},i}$ denotes the spacing error, with inter-vehicle distance $d_i = q_{i-1} - q_i - L_i$, vehicle's length $L_i$, and control gains ($k_p,k_d$). Define the follower and leader states $x_i = [d_i\, v_i\, a_i]^\top$ and $x\imo =[\vim \, \aim]^\top$, respectively. Substituting~\eqref{eq:SD_BaseController} into~\eqref{eq:PF_simplified_uncertain} yields the closed-loop system
\begin{align} \label{eq:CL_base_uncertain}
     & \hspace{-3mm} \begin{bmatrix}
        \dot{x}\imo\\ \dot x_i \\ \dot{{\rho}}_i
    \end{bmatrix} \!\!=\!\! 
    \begin{bmatrix}
        A^0_{i-1,i-1} & 0 & 0\\ 
        A^0_{i,i-1} & A^0_{i,i} &  B^0_{i,i} \\
        {B}^c_{i,i-1} & {B}^c_{i,i} & {A}^c_i 
    \end{bmatrix}\!\!
    \begin{bmatrix}
        x\imo \\ x_i \\ {\rho}_i
    \end{bmatrix} \nonumber \\ 
    & \hspace{-2mm} + \! \begin{bmatrix}
        (B^0_{i-1})^\top & 
        0     &
        (E^c_i)^\top     
    \end{bmatrix}^\top  
        \!\! \uim \! + \! 
    \begin{bmatrix}
        0 & 
        (B^\phi_i)^\top&
        0     
    \end{bmatrix}^\top  
        \!\! \phi_i,
\end{align}
where superscripts $0$ and $c$ indicate the nominal and controller matrices, respectively, given in Appendix~\ref{app:appendix1}. The base controller~\eqref{eq:SD_BaseController} achieves the desired tracking performance for~\eqref{eq:desiredModel} (i.e., $\phi_i = \Delta = 0$). However, for the true closed-loop system~\eqref{eq:CL_base_uncertain}, performance degradation occurs due to $\phi_i$.

To enhance robustness of~\eqref{eq:CL_base_uncertain} without altering the nominal closed-loop behavior, we exploit PEC realizations~\cite{huisman_optimal_2024,huisman_plant_2025}, i.e., distinct realizations producing the same control input $u_i$ in the nominal case while modifying the internal controller dynamics. To obtain the PEC realization of~\eqref{eq:SD_BaseController}, define a new controller state $\bar{\rho}_i$ via the linear transformation~\cite{huisman_optimal_2024,huisman_plant_2025}: 
\begin{align} \label{eq:PEC_Transformation}
  \!\!\! \bar{\rho}_i =  \rho_i + F_{i,i} x_i + F_{i,i-1} x\imo,
\end{align} 
where $F_{i,i} \in \mathbb{R}^{1\times 3}$ and $F_{i,i-1} \in \mathbb{R}^{1\times 2}$. To preserve the CACC information structure, explicit dependencies on vehicle $i-2$ are excluded by omitting $d_{i-1}$ in \eqref{eq:PEC_Transformation}. 

Differentiating~\eqref{eq:PEC_Transformation} and substituting the nominal dynamics~\eqref{eq:desiredModel} and~\eqref{eq:SD_BaseController} yields the PEC realization
\begin{subequations}\label{eq:PEC_Controller} \begin{align} \vspace{-3mm} \hspace{-2mm}
    \bar{\mathcal{F}} &\coloneqq \left\{
    \begin{aligned}
        \dot{\bar{\rho}}_i &= \bar{A}^c_i \bar{\rho}_i + \bar{B}^c_{i,i} x_i + \bar{B}^c_{i,i-1} x\imo + \bar{E}^c_i \uim, \\
        u_i &= \bar{\rho}_i - F_{i,i} x_i - F_{i,i-1} x\imo,
    \end{aligned} \right.          
\end{align}
with 
\begin{align}
    \bar{A}^c_i &= A_i^c + F_{i,i} B^0_{i}, \quad {\bar{E}}^c_i = E^c_i + F_{i,i-1} B^0_{i-1}\\
    \hspace{-2mm} \bar B^c_i &= B^c_i + F_{i,i} A^0_{i,i} - F_{i,i} B^0_{i,i} F_{i,i}- A^c_i F_{i,i}, \\
    \hspace{-2mm} {\bar{B}}^c_{i,i-1} &= {B}^c_{i,i-1} + F_{i,i-1} A^0_{i-1,i-1} + F_{i,i} A^0_{i,i-1} \nonumber \\
    & \qquad - F_{i,i} B^0_{i,i} F_{i,i-1} - A^c_i F_{i,i-1}. 
\end{align}
\end{subequations}
While the base controller~\eqref{eq:SD_BaseController} guarantees nominal performance by design~\cite{ploeg_design_2011,lefeber_cooperative_2020}, its internal realization is not unique which is observed in the PEC realization~\eqref{eq:PEC_Controller}. This non-uniqueness can be exploited to improve robustness without altering the nominal behavior.

Therefore, the problem addressed in this paper is to determine a PEC realization that improves the robustness of a CACC-controlled vehicle in the presence of parametric uncertainty. Specifically, given the base
controller~\eqref{eq:SD_BaseController}, we seek a PEC realization of the form~\eqref{eq:PEC_Controller}, by selecting the realization matrices $F_{i,i}$ and $F_{i,i-1}$, such that the influence of the uncertainty $\phi_i$ on~\eqref{eq:CL_base_uncertain} is minimized, aiming to preserve the nominal closed-loop behavior.
 


\begin{comment}
Substituting~\eqref{eq:SD_BaseController} into~\eqref{eq:PF_simplified_uncertain} yields the closed-loop system
\begin{subequations} \label{eq:CL_base_uncertain} \begin{multline} 
    \hspace{-4mm}\begin{bmatrix}
        \dot{x}\imo\\ \dot x_i \\ \dot{{\rho}}_i
    \end{bmatrix} \!\!=\!\! 
    \begin{bmatrix}
        A^0_{i-1,i-1} & 0 & 0\\ 
        A^0_{i,i-1} & A^0_{i,i} &  B^0_{i,i} \\
        {B}^c_{i,i-1} & {B}^c_{i,i} & {A}^c_i 
    \end{bmatrix}\!\!
    \begin{bmatrix}
        x\imo \\ x_i \\ {\rho}_i
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B^0_{i-1} \\ 
        0     \\
        E^c_i     
    \end{bmatrix}  
        \uim + 
    \begin{bmatrix}
        0 \\ 
        B^\phi_i  \\
        0     
    \end{bmatrix}  
        \phi_i,
\end{multline}
with
\begin{align}
    %%% Lead %%%
    \hspace{-2mm}A^0_{i-1,i-1} \!\!&=\!\!
    \begin{bmatrix}
        0 & 1 \\
        0 & - \frac{1}{\tau\imo}
    \end{bmatrix}\!\!, 
    A^0_{i,i-1} \!\!=\!\! 
    \begin{bmatrix}
        1 & 0 \\
        0 & 0 \\
        0 & 0
    \end{bmatrix}\!\!, 
    B^0_{i-1} \!=\! \begin{bmatrix}
        0 \\ \frac{1}{\tau\imo}, \\
    \end{bmatrix}\!\!, \\
     %%% Follower %%%
    \hspace{-2mm} A^0_{i,i} &= 
    \begin{bmatrix}
        0 & -1 & 0 \\
        0 & 0 & 1 \\
        0 & 0 & - \frac{1}{\tau_i}
    \end{bmatrix}\!, 
    B^0_i = \begin{bmatrix}
        0 \\ 0 \\ \frac{1}{\tau_i}, \\
    \end{bmatrix}\!,
    B^\phi_i \! = \! \begin{bmatrix}
        0 \\ 0 \\ 1 \\
    \end{bmatrix},\\
    A^c_i &=  -\tfrac{1}{h_i}, \quad
    B^c_{i,i-1} = \begin{bmatrix} \frac{k_d}{h_i} + \tfrac{\tau\imo - \tau_i}{h_i \tau\imo}& 0 \end{bmatrix}, \\
    B^c_{i,i}  &= \begin{bmatrix} \frac{k_p}{h_i} & -\left(k_p + \frac{k_d}{h_i}\right) & -k_d \end{bmatrix}, E^c = \tfrac{\tau_i}{h_i \tau\imo}, 
\end{align} \end{subequations}
where superscripts $0$ and $c$ indicate the nominal and controller matrices, respectively.

    with $f_{i,j}\in \mathbb{R},\,j\in\{1,...,6\}$, and $x_i = [d_i\, v_i\, a_i]^\top$ and $x\imo =[d\imo \, \vim \, \aim]^\top$ denoting the follower and leader states, respectively. Restricting the PEC realizations such that they are independent of $\tau\imo$, we take inspiration from~\cite{lefeber_cooperative_2020} and set $f_{i,6} = -\tfrac{\tau_i}{h_i}$. Furthermore, we set $f_{i,4}=0$ to avoid explicit dependencies between vehicles $i$ and $i-2$, which allows us to redefine $x\imo \coloneqq [\vim \, \aim]^\top$. 
\end{comment}


==> 3_ProblemSetting/3.2_ControllerRealizations.tex <==

\subsection{Plant Equivalent Controller Realization}
Consider the the states $x_1 = [v_1 \, a_1]^\top$ and $x_2 = [d_2\, v_2 \, a_2]^ \top$ with nominal (i.e., $\Delta = 0$) platooning dynamics
\begin{subequations} \label{eq:plantGeneral} \begin{align} \begin{aligned}
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2
    \end{bmatrix} &= 
    \begin{bmatrix}
        A_0^1               & \BO \\
        \tilde A_0^{2}      & A_0^2 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 
    \end{bmatrix} +  
    \begin{bmatrix}
        B_0^1   & \BO \\ 
        \BO     & B_0^2  
    \end{bmatrix}  
    \begin{bmatrix}
        u_1 \\ u_2 
    \end{bmatrix},
\end{aligned} \end{align}
with
\begin{align}
    %%% Lead %%%
    A_0^1 &= 
    \begin{bmatrix}
        0 & 1 \\
        0 & - \frac{1}{\tau_{\text{des}}}
    \end{bmatrix}, 
    \tilde A_0^2 = 
    \begin{bmatrix}
        1 & 0 \\
        0 & 0 \\
        0 & 0
    \end{bmatrix}, 
    B_0^1 = \begin{bmatrix}
        0 \\ \frac{1}{\tau_{\text{des}}}, \\
    \end{bmatrix}, \\
     %%% Follower %%%
    A_0^2 &= 
    \begin{bmatrix}
        0 & -1 & 0 \\
        0 & 0 & 1 \\
        0 & 0 & - \frac{1}{\tau_{\text{des}}}
    \end{bmatrix}, 
    B_0^2 = \begin{bmatrix}
        0 \\ 0 \\ \frac{1}{\tau_{\text{des}}}, \\
    \end{bmatrix}.
\end{align} \end{subequations}
To obtain the desired nominal performance, we consider the CACC scheme, which is considered the base controller, and is given by
\begin{align} \label{eq:BG_baseController}
    \dot u_2 &= -\frac{1}{h} u_2 + \frac{k_p}{h} e_2 + \frac{k_d}{h} \dot e_2 + \frac{1}{h} u_1,
\end{align}
with tracking error $e_2~\coloneqq d_2 - d_{r,i}$, where the goal is to follow a reference $d_{r,i} \coloneqq r_2 + h v_2$. Moreover, we have that $\dot e_2 \coloneqq \vim - v_2 - h a_2$. The base controller can be reformulated into a generic dynamic output feedback form
\begin{subequations}\label{eq:baseGeneral} \begin{align} 
    \dot{\rho}_2 &= A_c^i \rho_2 + B_{c}^i x_2 + \tilde B_c^{i-1} x_1 + \tilde E_c^{i-1} \uim, \\
    u_2 &= C_c^i \rho_2 + D_c^i x_2 + \tilde D_c^{i-1} x_1.
\end{align}
where the base controller is obtained for
\begin{align}
    \hspace{-3mm} A_c &= -\frac{1}{h}, && C_c = 1, \\
    \hspace{-3mm} \tilde B_c &= \begin{bmatrix} \frac{k_d}{h} & 0 \end{bmatrix}, && \tilde{D}_c =  \begin{bmatrix}  0 & 0  \end{bmatrix},\\
    \hspace{-3mm}B_c &=  \begin{bmatrix} \frac{k_p}{h} & -\left(k_p + \frac{k_d}{h}\right) & -k_d \end{bmatrix}, && D_c^i =  \begin{bmatrix} 0 & 0 & 0 \end{bmatrix}, \\
    \hspace{-3mm} \tilde E_c &= \frac{1}{h}.
\end{align} \end{subequations}
A class of plant equivalent controller (PEC) realizations of the base controller~\eqref{eq:baseGeneral} for plant~\eqref{eq:plantGeneral} is obtained via the linear change of coordinates
\begin{align} \label{eq:changeOfCoordinates}
    \bar \rho_2 = \rho_2 + F x_2 + \tilde F  x_1,
\end{align}
resulting in
\begin{subequations}\label{eq:BG_eqController} \begin{align} 
    \dot {\bar \rho}_2 &= \bar{A}_c \bar\rho_2 + \bar B_c x_2 + \tilde{\bar{B}}_c x_{1} +  
    \bar{E}_c u_{1}  \\
    u_2 &= \bar C_c \bar \rho_2 + \bar{D}_c x_2 + \tilde{\bar{D}}_c x_{1},
\end{align}
with
\begin{align}
    \hspace{-2mm} \bar{A}_c &= A_c + F B_0^2 C_c, \quad \bar C_c = C_c, \quad \bar D_c = D_c - C_c F,\\
    \hspace{-2mm} \bar B_c &= B_c + F A_0^2 + F B_0^2 (D_c - C_c F)- A_c F, \\
    \hspace{-2mm} \tilde{\bar{B}}_c &= \tilde{B}_c + \tilde F A_0^{1} + F \tilde A_0^{2} + F B_0^2(\tilde{D}_c - C_c \tilde F)- A_c \tilde F, \\
    \hspace{-2mm} \tilde{\bar{D}}_c &= \tilde{D}_c - C_c \tilde F, \qquad
    {\bar{E}}_c = E_c + \tilde F B_0^{1}.
\end{align}
\end{subequations}



==> 4_approach/4.1_closedLoop_V1.tex <==


Substituting the PEC realization~\eqref{eq:PEC_Controller} into the uncertain dynamics~\eqref{eq:PF_simplified_uncertain} yields the closed-loop system
\begin{multline} \label{eq:CL_PEC_uncertain} 
    \hspace{-4mm}\begin{bmatrix}
        \dot{x}_1\\ \dot x_2 \\ \dot{\bar{\rho}}_2
    \end{bmatrix} \!\!=\!\! 
    \begin{bmatrix}
        A^0_{1,1} & 0 & 0\\ 
        A^0_{2,1} - B^0_{2} F_{1} & A^0_{2,2} - B^0_{2} F_{2} &  B^0_{2} \\
        \bar{B}^c_{2,1} & \bar{B}^c_{2,2} & \bar{A}^c_2 
    \end{bmatrix}\!\!
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        (B^0_1)^\top  &
        0     &
        \bar{E}^c_2     
    \end{bmatrix}^\top  
        u_1 + 
    \begin{bmatrix}
        0 & 
        (B^\phi_2)^\top   &
        0     
    \end{bmatrix}^\top   
        \phi_2,
\end{multline}
where the corresponding system matrices are given in Appendix~\ref{app:appendix1}. By construction, the nominal closed-loop behavior of~\eqref{eq:CL_PEC_uncertain} is equivalent to that of ~\eqref{eq:CL_base_uncertain}, i.e., when $\Delta = \phi_2 = 0$. However, the choice of PEC realization matrix $F$ affects the closed-loop behavior in the presence of parametric uncertainty, i.e., when $\Delta \neq 0$ or, equivalently, $\phi_2 \neq 0$.

To explicitly characterize the influence of the  PEC realization, we rewrite the closed-loop dynamics~\eqref{eq:CL_PEC_uncertain} in the original controller coordinates $\rho_2$ by applying the inverse transformation of~\eqref{eq:PEC_Transformation}. In the case of uncertainties, this yields
\begin{align} \label{eq:CL_base_F}
    \hspace{-2mm}\begin{bmatrix}
        \dot{x}_1\\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} \!\! &=\!\! 
    \begin{bmatrix}
        A^0_{1,1} & 0 & 0\\ 
        A^0_{2,1} & A^0_{2,2} &  B^0_{2,2} \\
        {B}^c_{2,1} & {B}^c_{2,2} & {A}^c_2 
    \end{bmatrix}\!\!
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix}  \! +  \!
    \begin{bmatrix}
        B^0_1 \\
        0    \\
        E^c_2     
    \end{bmatrix}  
       u_1 \nonumber \\
        & \qquad + 
    \begin{bmatrix}
        0 &
        (B^\phi_2)^\top  &
        -F_{2} B^\phi_2     
    \end{bmatrix}^\top  
        \phi_2.
\end{align}

From~\eqref{eq:CL_base_F}, it is evident that the PEC realizations only affect the mapping of the uncertainty $\phi_2$ into the closed-loop dynamics. Moreover, this dependence occurs through the product $F_2 B^\phi_2$, which reduces to the scalar parameter $f_{2,3}$. Consequently, although $F \!\in \!\mathbb{R}^{1 \times 5}$, the effect of the PEC realization with respect to parametric uncertainty is fully characterized by the parameter $f_{2,3}$.

Since this result holds without imposing any assumptions on the structure of $\phi_2$, the remaining PEC parameters can be fixed without affecting robustness. In particular, inspired by~\cite{lefeber_cooperative_2020}, we choose $f_{1,2} = -\tfrac{\tau_i}{h_i}$, which yields PEC realizations that are independent of the leader input $u_1$ (i.e., $\bar{E}^c_2 = 0$) and driveline time constant $\tau_{i-1}$. The latter property is especially relevant for heterogeneous platoons, as it avoids dependency on the driveline dynamics of the preceding vehicle.

To determine $f_{2,3}$, we use Lemma~\ref{lemma1} and Lemma~\ref{lemma2}, corresponding to Quadratic Stability and the Bounded-Real Lemma for polytopic uncertain systems, respectively. To this end, the nonlinear uncertainty $\phi_2$ is approximated by a first-order Taylor expansion around an operating point $(v_i^*, a_i^*, u_i^*)$. We assume that both the leader and the follower vehicle travel at a constant reference velocity $v_{\mathrm{r}}$, yielding $(v_i^*, a_i^*, u_i^*) = (v_{\mathrm{r}}, 0, 0)$. Under this assumption, the closed-loop dynamics~\eqref{eq:CL_base_F} reduce to:
\begin{subequations} \label{eq:CL_uncertain2} 
\begin{align} 
    & \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} = \left(
    \begin{bmatrix}
        A^0_{1,1} & 0 & 0 \\ 
        A^0_{2,1} & A^0_{2,2} &  B^0_{2,2} \\
        {B}^c_{2,1} & {B}^c_{2,2} & {A}^c_2 
    \end{bmatrix} \right. \nonumber \\ & \left. + 
    \begin{bmatrix}
        0 & 0 & 0\\ 
        0 & A^\Delta_{2} & B^\Delta_{2} \\
        0 & -F_{2} A^\Delta_{2} & -F_{2} B^\Delta_{2} 
    \end{bmatrix} \right)
    \begin{bmatrix}
        x_1 \\ x_2 \\ \rho_2
    \end{bmatrix}  + 
    \begin{bmatrix}
        B^0_1 \\ 0 \\ 0
    \end{bmatrix} u_1 \nonumber \\ 
    & \,+ 
    \begin{bmatrix}
        0 & (B^\Delta_{0})^\top & -F_{2}B^\Delta_{0}
    \end{bmatrix}^\top
\end{align}
where substitution of~\eqref{eq:theta1}--\eqref{eq:theta6} yields
\begin{align} 
    \hspace{-2mm}A^\Delta_2 \hspace{-1mm}&=\hspace{-1mm} \sum_{j=1}^6 \! A^\Delta_{2,j} \Delta_j, \, B^\Delta_2 \hspace{-1mm}=\hspace{-1mm} \sum_{j=1}^6 \! B^\Delta_{2,j} \Delta_j, \,
    B^\Delta_0 \hspace{-1mm} = \hspace{-1mm} \sum_{j=1}^6 \!B^\Delta_{0,j} \Delta_j.
 \end{align}
\end{subequations}  
The matrices $A^\Delta_{2,j}, B^\Delta_{2,j}, B^\Delta_{0,j}$ are given in Appendix~\ref{app:uncertain}.

Define the uncertainty vector 
\begin{align}\begin{split}
    \Delta &\coloneqq 
    \begin{bmatrix}
        \Delta_1 & \Delta_2 & \Delta_3 & \Delta_4 & \Delta_5 & \Delta_6
    \end{bmatrix}^\top,     
\end{split}\end{align}
and the corresponding hyper-rectangle uncertainty set
\begin{align} \label{eq:uncertainConvexHull}
    \hspace{-3mm} \Delta \! \in \! \mathcal{D} := \left\{ \Delta \! \in \! \mathbb{R}^6 : \Delta_j \in [\underline{\Delta}_j, \overline{\Delta}_j], \; j \in \{1,\dots,6\} \right\}.
\end{align}

Since $A^\Delta_{2}, B^\Delta_{2}$, and $B^\Delta_{0}$ depend affinely on $\Delta_j$, their image over $\mathcal{D}$ lies in the convex hull of the matrices evaluated at the vertices of $\mathcal{D}$. There are $2^6$ vertices, corresponding to all binary combinations of lower and upper bounds. For each vertex $k=1,\dots,2^6$, let $v^{[k]} \in \{0,1\}^6$ indicate whether to use the lower ($v^{[k]}_j = 0$) or upper ($v^{[k]}_j = 1$) bound. Then
\begin{subequations}\begin{align}
    \Delta^{[k]}_j &= (1-v^{[k]}_j)\,\underline{\Delta}_j + v^{[k]}_j \,\overline{\Delta}_j, \\
     A^{\Delta|[k]}_{2} &= \sum_{j=1}^6 A^\Delta_{2,j} \Delta^{[k]}_j,  \quad
    B^{\Delta|[k]}_2 = \sum_{j=1}^6 B^\Delta_{2,j} \Delta^{[k]}_j, \\
    B^{\Delta|[k]}_0 &= \sum_{j=1}^6 B^\Delta_{0,j} \Delta^{[k]}_j, \qquad  \forall k\in \{1,...,2^p\}.
\end{align}\end{subequations}
Consequently, for any $\Delta \in \mathcal{D}$, the uncertain matrices belong to the polytope
\begin{subequations}\label{eq:uncertainPolytopic}\begin{align}
    \hspace{-2mm} A^\Delta_2 \!&=\! \sum_{k=1}^{2^6}\sum_{j=1}^6 \beta_k  A^\Delta_{2,j} \Delta^{[k]}_j, 
    \,\, B_2^\Delta \!=\! \sum_{k=1}^{2^6}\sum_{j=1}^6 \beta_k B^\Delta_{2,j} \Delta^{[k]}_j, \\
    \hspace{-2mm} B^\Delta_0 \!&=\! \sum_{k=1}^{2^p}\sum_{j=1}^p \beta_k  B^\Delta_{0,j} \Delta^{[k]}_j,     
    \quad \sum_{k=1}^{2^6} \beta_k \!= \!1, \quad \beta_k \geq 0. 
\end{align} \end{subequations}

Closed-loop system~\eqref{eq:CL_uncertain2} together  with~\eqref{eq:uncertainPolytopic} constitutes a polytopic uncertain system (Definition~\ref{def:polytopic_system}), which allows the use of Lemmas~\ref{lemma1} and~\ref{lemma2} to compute the optimal value of $f_{2,3}$. 


\begin{comment}

\begin{align}
     \hspace{-3mm} A^\Delta_{2} \! &= \!
     \begin{bmatrix}
        0 & 0 & 0 \\
        0 & 0 & 0 \\
        0 & \theta_{2,1} + 2 \theta_{2,3} v_r & \theta_{2,2} + \theta_{2,4} v_r  
     \end{bmatrix}, \\
     \!\! B^\Delta_{2} \! &= \!
     \begin{bmatrix}
        0 & 0 & \theta_{2,6} 
     \end{bmatrix}^\top\!\!\!, \,\, B^\Delta_{0} \! = \!
     \begin{bmatrix}
         0 & 0 & \theta_{2,5} - \theta_{2,3} v_r^2
     \end{bmatrix}^\top \!\!\!.  
\end{align} 


define the polytopic closed-loop system depending on the controller realization matrices $F^1$ and $F^2$ as
\begin{subequations}\label{eq:poly_ClosedLoop} \begin{align}
    \dot{\bar{\zeta}}_2 &= \bar{\mathcal{A}}_{\zeta_2} \bar{\zeta}_2 + \bar{\mathcal{B}}_{x_1} \tilde x_1  + \bar{\mathcal{B}}_{u_1}u_1 + \bar{\mathcal{B}}_{\omega^2}
\end{align}
where
\begin{align}
    \bar{\mathcal{A}}_{\zeta_2} &= \bar{\mathcal{A}}_{\zeta_2,0} + \bar{\mathcal{A}}_{\zeta_2,\Delta}, \quad 
    \bar{\mathcal{B}}_{x_1} = \bar{\mathcal{B}}_{x_1,0} + \bar{\mathcal{B}}_{x_1,\Delta}, \\
    \bar{\mathcal{A}}_{\zeta_2,0} &= \begin{bmatrix}
         A_0^2 + B_0^2 \bar D_c^2 & B_0^2 \bar C_c^2  \\
        \bar B_c^2 & \bar A_c^2  
    \end{bmatrix}, \quad 
   \bar{\mathcal{B}}_{x_1,0} = \begin{bmatrix}
        \tilde A_0^{2,1} + B_0^2  \tilde{\bar{D}}_c^1   \\
        \tilde{\bar{B}}^1_c  
    \end{bmatrix}, \\
    \bar{\mathcal{A}}_{\zeta_2,\Delta} &=     
     \begin{bmatrix}
        \sum_{k=1}^{2^p}\sum_{j=1}^p \beta_k \Delta^{[k]}_j \left( A^2_{\Delta,j} + B^2_{\Delta,j} \bar{D}_c^2\right) & \sum_{k=1}^{2^p}\sum_{j=1}^p \beta_k \Delta^{[k]}_j B^2_{\Delta,j} \bar{C}_c^2  \\
       \BO & 0 
    \end{bmatrix}, \\
    \bar{\mathcal{B}}_{x_1,\Delta} &= 
    \begin{bmatrix}
       \sum_{k=1}^{2^p}\sum_{j=1}^p \beta_k \Delta^{[k]}_j B^2_{\Delta,j} \tilde{\bar{D}}^1_c  \\
        0 
    \end{bmatrix}, \quad
    \bar{\mathcal{B}}_{\omega^2} = 
    \begin{bmatrix}
       \sum_{k=1}^{2^p}\sum_{j=1}^p \beta_k \Delta^{[k]}_j \omega^2_{\Delta,j}  \\
        0
    \end{bmatrix}.
\end{align} \end{subequations}



    \begin{multline}
    \tilde \phi_2(v_i, a_i, u_i) = \phi_2(v_i^*, a_i^*, u_i^*) 
    +\left. \frac{\partial \phi_2}{\partial v_i} \right|_{(v_i^*, a_i^*)} (v_i - v_i^*) \\
    +  \left. \frac{\partial \phi_2}{\partial a_i} \right|_{(v_i^*, a_i^*)} (a_i - a_i^*) 
    + \left. \frac{\partial \phi_2}{\partial u_i} \right|_{(v_i^*, a_i^*)} (u_i - u_i^*).
\end{multline}
i.e., $(v_i^*, a_i^*, u_i^*) = (v_{\mathrm{r}},0,0)$. Under this assumption, $\phi_2 \approx \tilde{\phi}_2$, where 
\begin{multline}
    \tilde \phi_2 = \left(\theta_{2,1} + 2 \theta_{2,3} v_r \right)v_2 + (\theta_{2,2} + \theta_{2,4} v_r)a_2 \\ + \theta_{2,6} u_2 - \theta_{2,3} v_r^2 + \theta_{2,5}.
\end{multline}


\end{comment}

==> 4_approach/4.2_optimalPEC_V1.tex <==
The objective is to derive the optimal PEC realization, i.e., the optimal value of $f_{2,3}$, such that the effect of the parametric uncertainty $\Delta$ on the closed-loop behavior is minimized. To this end, we employ Lemmas~\ref {lemma1} and~\ref {lemma2}, both of which require the system matrix $A$ to be Hurwitz. However, in~\eqref{eq:CL_uncertain2}, $A_{1,1}^0$ is not Hurwitz due to the uncontrolled leader, which introduces an integrator associated with the leader velocity. To circumvent this issue, the leader state $x_1$ is treated as an exogenous input, and the stability and performance analysis is restricted to the follower.

Furthermore, the leader is assumed to track a constant reference velocity $v_{\mathrm{r}}$, used as the operating point for linearizing $\phi_2$. This motivates the coordinate transformation $\!\tilde x_1 \!\! \coloneqq \! [\tilde v_1 \, a_1]^\top\!\!$, with $\tilde v_1 \! = \! v_1 \!\! - \! v_{\mathrm{r}}$, and we assume that $\tilde{x}_1  \!\in\! \mathcal{L}_2$.

Define the reduced closed-loop state $\zeta \coloneqq \begin{bmatrix} x_2^\top & \rho_2
\end{bmatrix}^\top$. Then, the closed-loop dynamics~\eqref{eq:CL_uncertain2} can be written as 
\begin{subequations} \label{eq:zeta_uncertain}
    \begin{align}
    \hspace{-3mm} \dot\zeta &= (\mathcal{A}^0 + \mathcal{A}^\Delta) \zeta + \mathcal{B}^0_1 \tilde{x}_1+ \mathcal{B}^\Delta_0, \\
    \hspace{-3mm} \mathcal{A}^0 &=     \begin{bmatrix}
        A^0_{2,2} &  B^0_{2} \\
        {B}^c_{2} & {A}^c_2 
    \end{bmatrix}, \quad \mathcal{A}^\Delta =    
    \begin{bmatrix}
        A^\Delta_{2} & B^\Delta_{2} \\
        -F_{2} A^\Delta_{2} & -F_{2} B^\Delta_{2} 
    \end{bmatrix}, \\
    \hspace{-3mm} \mathcal{B}^0_1 \!&=\! 
    \begin{bmatrix}
        (A^0_{2,1})^\top & {B}^c_{2,1} 
    \end{bmatrix}^\top, 
    \mathcal{B}^\Delta_0 \!=\!
    \begin{bmatrix}
        (B^\Delta_{0})^\top & -F_{2}B^\Delta_{0}
    \end{bmatrix}^\top\!\!\!.
\end{align}
\end{subequations}
The PEC design goal is to find $f_{2,3}$, embedded in $F_2$, to minimize the deviation of the uncertain closed-loop system~\eqref{eq:zeta_uncertain} from the desired nominal behavior. To quantify the deviation induced by the uncertainty, we introduce the nominal model
\begin{align}\label{eq:zeta_nominal}
    \dot\zeta^0 = \mathcal{A}^0 \zeta^0 + \mathcal{B}_1^0 \tilde x_1.
\end{align}
For $\Delta = 0$,~\eqref{eq:zeta_uncertain} reduces to~\eqref{eq:zeta_nominal}. Using the nominal model, we define the closed-loop error state $\zeta^e \coloneqq \zeta - \zeta^0$. Using~\eqref{eq:zeta_uncertain} and~\eqref{eq:zeta_nominal}, the error dynamics can be written as follows:
\begin{align}
    \dot\zeta_e = (\mathcal{A}^0 + \mathcal{A}^\Delta)\zeta_e
      + \mathcal{A}^\Delta \zeta_0
      + \mathcal{B}_0^\Delta.
\end{align}

Next, we define the stacked state $q \coloneqq \begin{bmatrix} \zeta_0^\top & \zeta_e^\top \end{bmatrix}^\top$, which evolves according to
\begin{align} \label{eq:qDyn}
    \dot q &=
    \underbrace{\begin{bmatrix}
        \mathcal{A}^0 & 0 \\
        \mathcal{A}^\Delta & \mathcal{A}^0 + \mathcal{A}^\Delta
    \end{bmatrix}}_{\mathcal{A}_q} q
    +
   \underbrace{\begin{bmatrix}
        \mathcal{B}_1^0 \\ 0
    \end{bmatrix}}_{\mathcal{B}_q} \tilde x_1
    +
    \begin{bmatrix}
        0 \\ \mathcal{B}_0^\Delta
    \end{bmatrix}.
\end{align}
This augmented system captures both the nominal closed-loop dynamics, represented by $\zeta^0$, and the deviation induced by the parametric uncertainty, represented by the error state $\zeta^e$. Since the uncertainty enters the dynamics through $\mathcal{A}^\Delta$, which depends linearly on $F_2$ (i.e., $f_{2,3}$), the system~\eqref{eq:qDyn} provides a suitable framework for quantifying and minimizing the impact of the parametric uncertainty $\Delta$ in platooning. 

Now, the design objective is twofold. First, we seek to reduce the influence of the nominal state $\zeta^0$ on the error state $\zeta^e$. This is achieved by minimizing $\mathrm{trace}(C_z P C_z^\top)$ in Lemma~\ref{lemma2}, thereby reducing the average energy of $\zeta^e$ in the output~\cite{boyd_linear_1994}. Second, since accurate tracking of the leader is a primary control objective of CACC, we aim to reduce the effect of the leader state $\tilde{x}_1$ on error $\zeta^e$. This motivates minimizing the worst-case amplification of $\tilde{x}_1$ to $\zeta^e$, hence minimizing $\gamma$ in Lemma~\ref{lemma2}.

To achieve this objective, we define the performance output $z$ as the error state
\begin{subequations}\label{eq:perfomanceOutput}
    \begin{align}
    z &\coloneqq  
    \begin{bmatrix}
        0 & C
    \end{bmatrix}q \eqqcolon C_zq, \\
    C &= \mathrm{diag}([1,1,1,0]).
\end{align}
\end{subequations}
Hence, we focus solely on the vehicle state $x_2$ rather than the controller state $\rho_2$. Consider the polytopic uncertain closed-loop system~\eqref{eq:uncertainPolytopic},~\eqref{eq:zeta_uncertain},~\eqref{eq:qDyn}, performance output~\eqref{eq:perfomanceOutput}, and uncertainty~\eqref{eq:uncertainConvexHull}. Based on Lemmas~\ref{lemma1} and~\ref{lemma2}, for a given $f_{2,3}$, if there exist a positive definite matrix $P \in \mathbb{R}^{8\times8}$ and a scalar $\gamma>0$, being the solution to the convex program: 
\begin{align} \label{eq:OP_OptProblem}
	\left\{
	\begin{aligned}
        &\underset{P, \gamma, f_{2,3}}{\min}
        && \mathrm{trace}(C_z P C_z^\top) + \gamma,\\
		&\text{\emph{s.t.}}
        && (\mathcal{A}_q)^\top P + P\mathcal{A}_q \prec 0,
        \quad k = 1,\ldots,2^6,\\
        &&&
        \begin{bmatrix}
			(\mathcal{A}_q)^\top P + P\mathcal{A}_q + C_z^\top C_z & P\mathcal{B}_q \\
			(\mathcal{B}_q)^\top P & -\gamma I
		\end{bmatrix}
        \preceq 0,
	\end{aligned}
	\right.
\end{align}
then the optimal value $f_{2,3}^*$ stabilizes the uncertain system while minimizing both the average output energy and worst-case amplification with respect to the leader states. This objective function reflects a trade-off between reducing error dynamic energy and suppressing leader-induced deviations, which is further discussed in the results section. 

Note that~\eqref{eq:OP_OptProblem} is solved via a line-search over $f_{2,3}$, as then the formulation reduces to an LMI. Future work will investigate reformulating the LMI to solve for $F_2$ directly, avoiding intensive grid searches as design degrees of freedom increase. The proposed optimization framework is experimentally validated, and the results are discussed in the subsequent section. 



\begin{comment}

\begin{align} \label{eq:OP_OptProblem}
	\left\{
	\begin{aligned}
        &\underset{P \succ 0,\, \gamma_q,\, f_{2,3}}{\min}
        && \mathrm{trace}(P) + \gamma_q,\\
		&\text{\emph{s.t.}}
        && (\mathcal{A}_q^{[k]})^\top P + P\mathcal{A}_q^{[k]} \prec 0,
        \quad k = 1,\ldots,2^6,\\
        &&&
        \begin{bmatrix}
			(\mathcal{A}_q^{[k]})^\top P + P\mathcal{A}_q^{[k]} + C_z^\top C_z & P\mathcal{B}_q^{[k]} \\
			(\mathcal{B}_q^{[k]})^\top P & -\gamma_q I
		\end{bmatrix}
        \preceq 0 ,
	\end{aligned}
	\right.
\end{align}
where $\mathcal{A}_q^{[k]}$ and $\mathcal{B}_q^{[k]}$ denote the closed-loop matrices evaluated at the $k$-th vertex of the uncertainty polytope.



Based on Lemmas~\ref{lemma1} and~\ref{lemma2}, the robust performance of the polytopic uncertain closed-loop system can be enforced by verifying the corresponding LMIs at all vertices of the uncertainty polytope. 
\begin{align} \label{eq:OP_OptProblem}
	\left\{\!\begin{aligned}
        &\underset{P,\gamma_2}{\min} \quad \text{trace}(P) + \gamma_q,\\
		&\text{\emph{s.t.}} \,\, P\succ0, \,  (\mathcal{A}^{[k]}_q)^\top \!P + P \mathcal{A}^{[k]}_q \prec 0, \, k=1,\ldots,2^6 \\
        & \begin{bmatrix}
			\left(\mathcal{A}^{[k]}_q\right)^\top P + P \mathcal{A}^{[k]}_q + C_z^\top C_z & P \mathcal{B}^{[k]}_q\\
			\left(\mathcal{B}^{[k]}_q\right)^\top P & -\gamma_q I         
	\end{bmatrix} \preceq 0,  
	\end{aligned}\right.
\end{align}

    Therefore, we define the desired closed-loop state $\zeta_2^0$, with dynamics
\begin{align}
        \dot{{\zeta}}_{0} &= \mathcal{A}^0 {\zeta}^0 + {\mathcal{B}}_{1}^0 \tilde x_1
\end{align}

Then, define the error between the uncertain model and the desired model $\zeta_2^e = \zeta_2 -\zeta_2^0$, with dynamics
\begin{align} \begin{split}
    \dot\zeta_2^e &= \mathcal{A}_{\zeta_2} {\zeta}_2 + {\mathcal{B}}_{x_1}^\Delta \tilde x_1  + {\mathcal{B}}_{\omega^2} - \mathcal{A}_{\zeta_2^0} {\zeta}_{2,0}
\end{split} \end{align}
substituting $\zeta_{2} = \zeta_2^0+\zeta_2^e$
\begin{align} \begin{split}
    \dot\zeta_2^e &= \mathcal{A}_{\zeta_2}\zeta_2^e + \mathcal{A}_{\zeta_2,\Delta} {\zeta}_{2,0} + {\mathcal{B}}_{x_1, \Delta} \tilde x_1  + {\mathcal{B}}_{\omega^2}.
\end{split} \end{align}

Define stacked state $q = [\zeta_2^0\, \zeta_2^e]^\top$ and performance output $z$ then
\begin{align}
    \dot {q} &= 
    \begin{bmatrix}
        \mathcal{A}_{\zeta_2^0} & \BO, \\
         \mathcal{A}_{\zeta_2,\Delta} & \mathcal{A}_{\zeta_2}
    \end{bmatrix} q + 
    \begin{bmatrix}
      \mathcal{B}_{x_{1,0}} \\ \mathcal{B}_{x_1, \Delta}
    \end{bmatrix} \tilde x_1 +
    \begin{bmatrix}
     \mathcal{B}_{u_1}   \\ \BO
    \end{bmatrix} u_1 + 
    \begin{bmatrix}
     \BO \\ \mathcal{B}_{\omega^2}
    \end{bmatrix}, \\
    z &= y - y_0 = C(\zeta_2 - \zeta_2^0) = 
    \begin{bmatrix}
        \BO & C
    \end{bmatrix} q.
\end{align}
\end{comment}




==> 4_vehicleModel/4.1_nonlinearModel.tex <==
\subsection{Nonlinear Vehicle Model}

To obtain an LTI system, we linearize the nonlinear system around an operating point $(v_i^*,a_i^*,u_i^*)$ using a first order taylor expansion
\begin{subequations} \begin{multline}
f_\Delta(v_i, a_i, u_i) \approx f_\Delta(v_i^*, a_i^*, u_i^*) 
+\left. \frac{\partial f_\Delta}{\partial v_i} \right|_{(v_i^*, a_i^*)} (v_i - v_i^*) \\
+  \left. \frac{\partial f_\Delta}{\partial a_i} \right|_{(v_i^*, a_i^*)} (a_i - a_i^*) 
+ \left. \frac{\partial f_\Delta}{\partial u_i} \right|_{(v_i^*, a_i^*)} (u_i - u_i^*),
\end{multline}
where
% Compute partial derivatives
 \begin{align}
    \left. \frac{\partial f_\Delta}{\partial v_i} \right|_{(v_i^*, a_i^*)} &= c_1 + 2 c_3 v_i^* + c_4 a_i^*,\\
    \left. \frac{\partial f_\Delta}{\partial a_i} \right|_{(v_i^*, a_i^*)} &= c_2 + c_4 v_i^*, \qquad 
    \left. \frac{\partial f_\Delta}{\partial u_i} \right|_{(v_i^*, a_i^*)} = c_6.
\end{align} \end{subequations}

We assume that the leader, and therefore also the follower vehicle, follows a steady-state reference velocity $v_{\text{r}}$, i.e., $v_i^* = v_{\text{r}}$ and $a_i^* = u_i^* = 0$, resulting in
\begin{multline}
        \dot{a}_i = \left( c_2 + c_4 v_{\text{r}} - \frac{1}{\tau_{\text{des}}}\right) a_i + \left(c_6 + \frac{1}{\tau_{\text{des}}}\right) u_i \\
        \left(c_1 + 2c_3 v_{\text{r}}\right) (v_i - v_{\text{r}}) + c_1 v_{\text{r}} + c_3 v_{\text{r}}^2 + c_5 \\
        = \left( c_2 + c_4 v_{\text{r}} - \frac{1}{\tau_{\text{des}}}\right) a_i + \left(c_6 + \frac{1}{\tau_{\text{des}}}\right) u_i \\
        \left(c_1 + 2c_3 v_{\text{r}}\right) v_i - c_3 v_{\text{r}}^2 + c_5.
\end{multline}


\begin{comment}
Consider the nonlinear vehicle model of the $i$th~\cite{sheikholeslam_longitudinal_1993,sahlholm_road_2010, alam_guaranteeing_2014,besselink_cyberphysical_2016}:
\begin{subequations}\label{eq:PF_NLModel}\begin{align}
    \dot{F}_{\text{drive},i} &= -\frac{F_{\text{drive},i}}{\tau_i} + \frac{\eta_i}{\tau_i}, \label{eq:PF_engDyn} \\
     m_{\text{eff},i} a_i &= F_{\text{drive,i}} - F_d - F_v - F_{r} - F_g, \label{eq:PF_accDyn}
\end{align}
where $m_{\text{eff},i}$ represents the effective vehicle mass, $F_{\text{drive},i}$ the driving force, $\eta_i$ the input to the engine, $F_d$ the aerodynamic drag, $F_v$ the viscous friction force, $F_r$ the roll friction force, and $F_g$ the gravitational force, which yield
\begin{align}   
    F_d &= C_d (v_i-v_w )^2, \qquad
    &&F_v = f_v v_i, \label{eq:PF_Forces} \\ 
    F_r &\approx f_r m_i g,  \,\,
    && F_g \approx m_i g \alpha.
\end{align}\end{subequations}
Here, $C_d$ denotes the drag coefficient, $v_w$ the wind speed, $f_v$ is the viscous friction coefficient, $f_r$ the roll friction coefficient, $m_i$ the mass of vehicle $i$, $g$ the gravitational constant, and $\alpha$ the road slope. 

Assuming that the average road slope is relatively small ($\alpha \approx 0$) and slow variations of $F_r$ and $F_g$, differentiation of \eqref{eq:PF_accDyn} and \eqref{eq:PF_Forces} yields
\begin{subequations}\begin{align}
    m_{\text{eff},i} \dot{a}_i &= \dot{F}_{\text{drive},i} - \dot{F}_d - \dot{F}_v, \\
    \dot{F}_d &= 2C_d(v_i a_i - v_w a_i), \qquad
    \dot{F}_v = f_v a_i.
\end{align}\end{subequations}
Working this out and substitution of~\eqref{eq:PF_engDyn} and~\eqref{eq:PF_accDyn} yields
\begin{multline} \label{eq:PF_nlPlatoon}
     \dot{a}_i = - \tfrac{f_v - 2C_d v_w}{\tau_i m_{\text{eff},i}} v_i - \left(\tfrac{f_v - 2C_d v_w}{m_{\text{eff},i}} + \tfrac{1}{\tau_i} \right)a_i -\tfrac{C_d}{\tau_i m_{\text{eff},i}}v_i^2 \\
    - \tfrac{2 C_d}{m_{\text{eff},i}}v_i a_i - \tfrac{m_i(f_r g + g \alpha) + C_d v_w^2}{\tau_i m_{\text{eff},i}} + \tfrac{1}{\tau_i m_{\text{eff},i}} \eta_i.
\end{multline}

In~\cite{sheikholeslam_longitudinal_1993,sahlholm_road_2010, alam_guaranteeing_2014,besselink_cyberphysical_2016}, the input-output linearization is achieved via $\eta_i$ in~\eqref{eq:PF_nlPlatoon}, however, knowing all the model parameters in~\eqref{eq:PF_nlPlatoon} exactly is quite a strong assumption. Therefore, we identify six parameter groups $p_j, \, j\in \{1,...,6\}$, each with an initial estimate $p_{j|0}$ and associated uncertainty $\Delta_j$, which allows us to rewrite \eqref{eq:PF_nlPlatoon} 
\begin{multline}\label{eq:PF_nl_Uncertain}
   \! \! \! \dot{a}_i =  -(p_{1|0} + \Delta_1)v_i - (p_{2|0} + \Delta_2)a_i -(p_{3|0} + \Delta_{3})v_i^2 \\ 
    - (p_{4|0} + \Delta_{4}) v_i a_i - (p_{5|0} + \Delta_5) + (p_{6|0} + \Delta_6) \eta_i.
\end{multline}
Input-Output linearization is then applied using the nominal parameter estimates $p_{j|0}$, and by defining the desired linear model $\tfrac{1}{\tau_\text{des}}(u_i-a_i)$ with new input $u_i$ (which will be the input from the CACC controller), yielding
\begin{multline} \label{eq:PF_IOcontroller_param}
        \eta_i =  p_{6|0}^{-1} \left(  p_{1|0} v_i + \left(p_{2|0} - \frac{1}{\tau_{\text{des}}}\right) a_i + p_{3|0} v^2_i \right. \\
        \left. + p_{4|0} v_i a_i + p_{5|0} + \frac{1}{\tau_{\text{des}}} u_i \right).
\end{multline}
Substituting \eqref{eq:PF_IOcontroller_param} in the uncertain model in \eqref{eq:PF_nl_Uncertain} yields
\begin{subequations} \label{eq:PF_simplified_uncertain} \begin{align}
    \dot{a}_i &= - \frac{1}{\tau_{\text{des}}} a_i + \frac{1}{\tau_{\text{des}}} u_i + d(v_i,a_i,u_i).
\end{align}
where
\begin{multline}
   d(v_i,a_i,u_i) = d_1 v_i + d_2 a_i + d_3  v_i^2  + d_4 v_i a_i \\ + d_5 + d_6  u_i,
\end{multline}
\begin{align}
    d_1 &= \frac{p_{1|0}}{p_{6|0}}\Delta_6 - \Delta_1, \\
    d_2 &= \left(\frac{p_{2|0}}{p_{6|0}} - \frac{1} {p_{6|0}\tau_{\text{des}}} \right) \Delta_6 - \Delta_2, \\
    d_3 &= \frac{p_{3|0}}{p_{6|0}}\Delta_6 - \Delta_3, \qquad
    d_4 = \frac{p_{4|0}}{p_{6|0}} \Delta_6 - \Delta_4, \\
    d_5 &= \frac{p_{5|0}}{p_{6|0}} \Delta_6 - \Delta_5, \qquad 
    d_6 = \frac{1}{p_{6|0}\tau_{\text{des}}} \Delta_6.
\end{align}
\end{subequations}
Here, $d(v_i,a_i,u_i)$ is a nonlinear function, depending on the vehicle states and the desired acceleration. 

\end{comment}

==> 4_vehicleModel/4.2_uncertainClosedLoop.tex <==
\subsection{Uncertain Closed-Loop Dynamics}
The closed-loop system \eqref{eq:plantGeneral}~\eqref{eq:baseGeneral} and \eqref{eq:plantGeneral}~\eqref{eq:BG_eqController} result in the same closed-loop behavior; however, this is not guaranteed when we consider model uncertainty, i.e., the open-loop dynamics in \eqref{eq:PF_simplified_uncertain}. 

\begin{subequations} \label{eq:CL_bar_uncertain} \begin{multline} 
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{\bar{\rho}}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        A_0^1               & 0 & 0\\ 
        \tilde A_0^{2} + B_0^2 \tilde{\bar{D}}_c & A_0^2 + B_0^2 \bar{D}_c &  B_0^2 \bar C_c \\
        \tilde{\bar{B}}_c & \bar B_c & \bar{A}_c 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B_0^1 \\ 
        0     \\
        \bar{E}_c     
    \end{bmatrix}  
        u_1 + 
    \begin{bmatrix}
        0 \\ 
        B^2_\Delta  \\
        0     
    \end{bmatrix}  
        f_\Delta(v_2, a_2, u_2),
\end{multline}
with
\begin{align}
    B_\Delta^2 = \begin{bmatrix}
        0 \\ 0 \\ 1
    \end{bmatrix}.
\end{align}\end{subequations}

Note that the proposed change of coordinates in \eqref{eq:changeOfCoordinates} can be viewed as a change of coordinates on the closed-loop states of the following form
\begin{multline} \label{eq:inverseChangeCoordinates}
    \begin{bmatrix}
        x_1 \\x_2 \\ \bar{\rho}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        I & 0 & 0\\ 
        0 & I & 0 \\
        \tilde F & F & 1 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \rho_2
    \end{bmatrix} \iff \\
    \begin{bmatrix}
        x_1 \\x_2 \\ \rho_2
    \end{bmatrix} = 
    \begin{bmatrix}
        I & 0 & 0\\ 
        0 & I & 0 \\
        -\tilde F & -F & 1 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix}.
\end{multline}

Hence, we can convert~\eqref{eq:CL_bar_uncertain} back to the original controller state $\rho$ by applying~\eqref{eq:inverseChangeCoordinates} to obtain
\begin{multline} \label{eq:CL_uncertain} 
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        A_0^1               & 0 & 0\\ 
        \tilde A_0^{2} + B_0^2 \tilde{{D}}_c & A_0^2 + B_0^2 {D}_c &  B_0^2  C_c \\
        \tilde{{B}}_c &  B_c & {A}_c 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ {\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B_0^1 \\ 
        0     \\
        {E}_c     
    \end{bmatrix}  
        u_1 + 
    \begin{bmatrix}
        0 \\ 
        B^2_\Delta  \\
        0     
    \end{bmatrix}  
        f_\Delta,
\end{multline} 


\subsection{PART 2?}
\subsection{Plant Equivalent Controller Realization}
Consider the the states $x_1 = [v_1 \, a_1]^\top$ and $x_2 = [d_2\, v_2 \, a_2]^ \top$ with nominal (i.e., $\Delta = 0$) platooning dynamics
\begin{subequations} \label{eq:plantGeneral} \begin{align} \begin{aligned}
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2
    \end{bmatrix} &= 
    \begin{bmatrix}
        A_0^1               & \BO \\
        \tilde A_0^{2}      & A_0^2 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 
    \end{bmatrix} +  
    \begin{bmatrix}
        B_0^1   & \BO \\ 
        \BO     & B_0^2  
    \end{bmatrix}  
    \begin{bmatrix}
        u_1 \\ u_2 
    \end{bmatrix},
\end{aligned} \end{align}
with
\begin{align}
    %%% Lead %%%
    A_0^1 &= 
    \begin{bmatrix}
        0 & 1 \\
        0 & - \frac{1}{\tau_{\text{des}}}
    \end{bmatrix}, 
    \tilde A_0^2 = 
    \begin{bmatrix}
        1 & 0 \\
        0 & 0 \\
        0 & 0
    \end{bmatrix}, 
    B_0^1 = \begin{bmatrix}
        0 \\ \frac{1}{\tau_{\text{des}}}, \\
    \end{bmatrix}, \\
     %%% Follower %%%
    A_0^2 &= 
    \begin{bmatrix}
        0 & -1 & 0 \\
        0 & 0 & 1 \\
        0 & 0 & - \frac{1}{\tau_{\text{des}}}
    \end{bmatrix}, 
    B_0^2 = \begin{bmatrix}
        0 \\ 0 \\ \frac{1}{\tau_{\text{des}}}, \\
    \end{bmatrix}.
\end{align} \end{subequations}
To obtain the desired nominal performance, we consider the CACC scheme, which is considered the base controller, and is given by
\begin{align} \label{eq:BG_baseController}
    \dot u_2 &= -\frac{1}{h} u_2 + \frac{k_p}{h} e_2 + \frac{k_d}{h} \dot e_2 + \frac{1}{h} u_1,
\end{align}
with tracking error $e_2~\coloneqq d_2 - d_{r,i}$, where the goal is to follow a reference $d_{r,i} \coloneqq r_2 + h v_2$. Moreover, we have that $\dot e_2 \coloneqq \vim - v_2 - h a_2$. The base controller can be reformulated into a generic dynamic output feedback form
\begin{subequations}\label{eq:baseGeneral} \begin{align} 
    \dot{\rho}_2 &= A_c^i \rho_2 + B_{c}^i x_2 + \tilde B_c^{i-1} x_1 + \tilde E_c^{i-1} \uim, \\
    u_2 &= C_c^i \rho_2 + D_c^i x_2 + \tilde D_c^{i-1} x_1.
\end{align}
where the base controller is obtained for
\begin{align}
    \hspace{-3mm} A_c &= -\frac{1}{h}, && C_c = 1, \\
    \hspace{-3mm} \tilde B_c &= \begin{bmatrix} \frac{k_d}{h} & 0 \end{bmatrix}, && \tilde{D}_c =  \begin{bmatrix}  0 & 0  \end{bmatrix},\\
    \hspace{-3mm}B_c &=  \begin{bmatrix} \frac{k_p}{h} & -\left(k_p + \frac{k_d}{h}\right) & -k_d \end{bmatrix}, && D_c^i =  \begin{bmatrix} 0 & 0 & 0 \end{bmatrix}, \\
    \hspace{-3mm} \tilde E_c &= \frac{1}{h}.
\end{align} \end{subequations}
A class of plant equivalent controller (PEC) realizations of the base controller~\eqref{eq:baseGeneral} for plant~\eqref{eq:plantGeneral} is obtained via the linear change of coordinates
\begin{align} \label{eq:changeOfCoordinates}
    \bar \rho_2 = \rho_2 + F x_2 + \tilde F  x_1,
\end{align}
resulting in
\begin{subequations}\label{eq:BG_eqController} \begin{align} 
    \dot {\bar \rho}_2 &= \bar{A}_c \bar\rho_2 + \bar B_c x_2 + \tilde{\bar{B}}_c x_{1} +  
    \bar{E}_c u_{1}  \\
    u_2 &= \bar C_c \bar \rho_2 + \bar{D}_c x_2 + \tilde{\bar{D}}_c x_{1},
\end{align}
with
\begin{align}
    \hspace{-2mm} \bar{A}_c &= A_c + F B_0^2 C_c, \quad \bar C_c = C_c, \quad \bar D_c = D_c - C_c F,\\
    \hspace{-2mm} \bar B_c &= B_c + F A_0^2 + F B_0^2 (D_c - C_c F)- A_c F, \\
    \hspace{-2mm} \tilde{\bar{B}}_c &= \tilde{B}_c + \tilde F A_0^{1} + F \tilde A_0^{2} + F B_0^2(\tilde{D}_c - C_c \tilde F)- A_c \tilde F, \\
    \hspace{-2mm} \tilde{\bar{D}}_c &= \tilde{D}_c - C_c \tilde F, \qquad
    {\bar{E}}_c = E_c + \tilde F B_0^{1}.
\end{align}
\end{subequations}

\subsection{Uncertain Closed-Loop Dynamics}
The closed-loop system \eqref{eq:plantGeneral}~\eqref{eq:baseGeneral} and \eqref{eq:plantGeneral}~\eqref{eq:BG_eqController} result in the same closed-loop behavior; however, this is not guaranteed when we consider model uncertainty, i.e., the open-loop dynamics in \eqref{eq:PF_simplified_uncertain}. 

\begin{subequations} \label{eq:CL_bar_uncertain} \begin{multline} 
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{\bar{\rho}}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        A_0^1               & 0 & 0\\ 
        \tilde A_0^{2} + B_0^2 \tilde{\bar{D}}_c & A_0^2 + B_0^2 \bar{D}_c &  B_0^2 \bar C_c \\
        \tilde{\bar{B}}_c & \bar B_c & \bar{A}_c 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B_0^1 \\ 
        0     \\
        \bar{E}_c     
    \end{bmatrix}  
        u_1 + 
    \begin{bmatrix}
        0 \\ 
        B^2_\Delta  \\
        0     
    \end{bmatrix}  
        f_\Delta(v_2, a_2, u_2),
\end{multline}
with
\begin{align}
    B_\Delta^2 = \begin{bmatrix}
        0 \\ 0 \\ 1
    \end{bmatrix}.
\end{align}\end{subequations}

Note that the proposed change of coordinates in \eqref{eq:changeOfCoordinates} can be viewed as a change of coordinates on the closed-loop states of the following form
\begin{multline} \label{eq:inverseChangeCoordinates}
    \begin{bmatrix}
        x_1 \\x_2 \\ \bar{\rho}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        I & 0 & 0\\ 
        0 & I & 0 \\
        \tilde F & F & 1 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \rho_2
    \end{bmatrix} \iff \\
    \begin{bmatrix}
        x_1 \\x_2 \\ \rho_2
    \end{bmatrix} = 
    \begin{bmatrix}
        I & 0 & 0\\ 
        0 & I & 0 \\
        -\tilde F & -F & 1 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ \bar{\rho}_2
    \end{bmatrix}.
\end{multline}

Hence, we can convert~\eqref{eq:CL_bar_uncertain} back to the original controller state $\rho$ by applying~\eqref{eq:inverseChangeCoordinates} to obtain
\begin{multline} \label{eq:CL_uncertain} 
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        A_0^1               & 0 & 0\\ 
        \tilde A_0^{2} + B_0^2 \tilde{{D}}_c & A_0^2 + B_0^2 {D}_c &  B_0^2  C_c \\
        \tilde{{B}}_c &  B_c & {A}_c 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ {\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B_0^1 \\ 
        0     \\
        {E}_c     
    \end{bmatrix}  
        u_1 + 
    \begin{bmatrix}
        0 \\ 
        B^2_\Delta  \\
        -F B^2_\Delta    
    \end{bmatrix}  
        f_\Delta,
\end{multline} 

\begin{multline}
        f_\Delta = 
    \begin{bmatrix}
        0 & c_1+2c_3v_r & c_2+c_4 v_r
    \end{bmatrix} x_2 \\ + c_6 u_2 + c_5-c_3v_r^2  
\end{multline}


\begin{multline} \label{eq:CL_uncertain2} 
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} = 
    \left( \begin{bmatrix}
        0 & 1 & 0 & 0 & 0 & 0 \\ 
        0 & -\tfrac{1}{\tau_{\text{des}}} & 0 & 0 & 0 & 0\\
        1 & 0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 0 & -\tfrac{1}{\tau_{\text{des}}} & \tfrac{1}{\tau_{\text{des}}} \\
        \tfrac{k_d}{h} & 0 & \tfrac{k_p}{h} & -(k_p + \tfrac{k_d}{h})& -k_d & -\tfrac{1}{h}  
        \end{bmatrix}
    \right. \\ \left. 
    \begin{bmatrix}
        0 & 0 & 0 & 0 & 0 & 0 \\ 
        0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & c_1 + 2c_3 v_r & c_2 + c_4 v_r & c_6 \\
        0 & 0 & 0 & F_3(c_1 + 2c_3 v_r) & F_3(c_2 + c_4 v_r) & F_3 c_6
        \end{bmatrix}
        \right)     \begin{bmatrix}
        v_1 \\ a_1 \\ d_2 \\ v_2 \\ a_2 \\ {\rho}_2
    \end{bmatrix} \\
    +  
    \begin{bmatrix}
        0 \\ \frac{1}{\tau_{\text{des}}} \\
        0 \\ 0 \\ 0 \\
        \frac{1}{h}    
    \end{bmatrix}  
        u_1 +  
    \begin{bmatrix}
        0 \\ 0 \\
        0 \\ 0 \\ c_5 - c_3 v_r^2 \\
       F_3(c_5 - c_3 v_r^2)
    \end{bmatrix}  
\end{multline} 



==> 5.Optimization.tex <==


\section{Optimal PEC Realization} \label{sec:Results} \vspace{-1mm}
TBD



==> 5.Optimization/5.1_ErrorDynamics.tex <==
\subsection{Error Dynamics}

Define $q = [\zeta_{2,0}, \, \zeta_{2,e}]$, with $\zeta_2 = [x_2, \rho_2]$

\begin{multline}  
    \begin{bmatrix}
        \dot x_1 \\ \dot x_2 \\ \dot{{\rho}}_2
    \end{bmatrix} = 
    \begin{bmatrix}
        A_0^1               & 0 & 0\\ 
        \tilde A_0^{2} + B_0^2 \tilde{{D}}_c & A_0^2 + B_0^2 {D}_c &  B_0^2  C_c \\
        \tilde{{B}}_c &  B_c & {A}_c 
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ x_2 \\ {\rho}_2
    \end{bmatrix} \\ +  
    \begin{bmatrix}
        B_0^1 \\ 
        0     \\
        {E}_c     
    \end{bmatrix}  
        u_1 + 
    \begin{bmatrix}
        0 \\ 
        B^2_\Delta  \\
        -F B^2_\Delta    
    \end{bmatrix}  
        f_\Delta,
\end{multline} 


\begin{subequations}
\begin{align}
\begin{split}
        \dot \zeta &= (\mathcal{A}_{0} + S^{-1} \mathcal{A}_\Delta)\zeta \\ 
        & \qquad \qquad + (\mathcal{B}_{0} + S^{-1}\mathcal{B}_{\Delta}) \begin{bmatrix}
        x_1 \\ u_1
        \end{bmatrix} + S^{-1}\mathcal{B}_\omega,
\end{split} \\
    \dot \zeta_0 &= \mathcal{A}_{0} \zeta_0 + \mathcal{B}_{0} \begin{bmatrix}
        x_1 \\ u_1
    \end{bmatrix} 
\end{align}
define $\zeta_e = \zeta - \zeta_0$, with dynamics
\begin{align}
    \dot \zeta_e &= \dot\zeta - \dot\zeta_0, \\
    \begin{split}
        &= (\mathcal{A}_{0} + S^{-1} \mathcal{A}_\Delta)\zeta + (\mathcal{B}_{0} + S^{-1}\mathcal{B}_{\Delta}) \begin{bmatrix}
        x_1 \\ u_1
    \end{bmatrix} \\
    &\quad + S^{-1}\mathcal{B}_\omega - \left( \mathcal{A}_{0} \zeta_0 + \mathcal{B}_{0} \begin{bmatrix}
        x_1 \\ u_1 \end{bmatrix} \right)
    \end{split} \\
    \begin{split}
        &= (\mathcal{A}_{0} + S^{-1} \mathcal{A}_\Delta)\zeta_e + S^{-1} \mathcal{A}_\Delta \zeta_0 \\ &\quad + S^{-1}\mathcal{B}_{\Delta} \begin{bmatrix}
        x_1 \\ u_1
    \end{bmatrix}  + S^{-1}\mathcal{B}_\omega 
    \end{split} 
\end{align}
\end{subequations}

\begin{subequations}\begin{multline}
    \begin{bmatrix}
        \dot \zeta_0 \\ \dot \zeta_e
    \end{bmatrix} = 
    \begin{bmatrix}
       \mathcal{A}_0 & 0 \\
       S^{-1} \mathcal{A}_\Delta &  (\mathcal{A}_{0} + S^{-1} \mathcal{A}_\Delta)
    \end{bmatrix}
    \begin{bmatrix}
        \zeta_0 \\ \zeta_e
    \end{bmatrix} \\ +
    \begin{bmatrix}
        \mathcal{B}_0 \\
        S^{-1}\mathcal{B}_{\Delta}
    \end{bmatrix}
    \begin{bmatrix}
        x_1 \\ u_1
    \end{bmatrix}
    + 
    \begin{bmatrix}
       0 \\  S^{-1}\mathcal{B}_\omega
    \end{bmatrix}
\end{multline}
with performance output $z$ defined as
\begin{align}
    z &= y - y_0 = C (\zeta - \zeta_0) = C \zeta_e, \\
    C &= \text{diag}[1,1,1,0].
\end{align}\end{subequations}

Define $q = \begin{bmatrix}\zeta_0^\top & \zeta_e^\top\end{bmatrix}^\top$, and via the bounded real-lemma we obtain
\begin{align}
    \begin{bmatrix}
        \mathcal{A}_q^\top P + P \mathcal{A}_q + C_q^\top C_q & P \mathcal{B}_q \\ 
    \mathcal{B}_q^\top P & -\gamma^2 I 
    \end{bmatrix} \leq 0
\end{align}

==> 5.Optimization/5.2_optimizationProblem.tex <==
\subsection{Optimization Formulation}

==> 6.Results/6.1_simulation.tex <==
TBD


==> 6.Results_V1.tex <==
\section{Case Study Results} \label{sec:Results} \vspace{-2mm}
This section presents the results obtained by solving the optimization problem~\eqref{eq:OP_OptProblem}. The objective of~\eqref{eq:OP_OptProblem} is to enhance the robustness of the uncertain closed-loop system~\eqref{eq:CL_base_uncertain} with respect to $\phi_2$, i.e., $\Delta$, while preserving the desired closed-loop behavior. Both the simulation study and the experimental validation are conducted using the vehicle parameters and associated uncertainties listed in TABLE~\ref{tab:vehicle_params}. The optimization problem is solved in MATLAB~2025b using YALMIP~\cite{lofberg_yalmip_2004}, with solver MOSEK~\cite{mosek_aps_mosek_2024}.
\begin{table}[bt]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Vehicle Parameters and estimated uncertainties of the Renault Twizy test platform.}
\label{tab:vehicle_params} \vspace{-2mm}
\begin{tabular}{llccc}
\toprule
\textbf{Sym.} & \textbf{Parameter} & \textbf{Nominal} & \textbf{Range ($\Delta$)} & \textbf{Unit} \\ 
\midrule
$m$              & Vehicle Mass          & 731    & $[716, 746]$       & kg \\
$m_{\text{eff}}$ & Effective Mass        & 778    & $[763, 793]$       & kg \\
$f_v$            & Viscous Friction      & 5.55   & $[5.5, 5.6]$       & Ns/m \\
$f_r$            & Rolling Res. Coeff.   & 0.0262 & $[0.0262, 0.0262]$ & -- \\
$C_d$            & Aero. Drag Factor     & 0.392  & $[0.3528, 0.4312]$ & kg/m \\
$\tau$           & Time Constant         & 0.12   & $[0.11, 0.13]$     & s \\
$\alpha$         & Road Slope            & 0      & $[0, 0]$           & rad \\
$v_{\text{w}}$& Wind Velocity         & 0      & $[-5, 5]$          & m/s \\
$k_p$            & Proportional gain     & 0.2    & --                 & 1/s$^2$ \\ 
$k_d$            & Derivative gain       & 0.7    & --                 & 1/s \\ 
$h$              & Headway time          & 0.2    & --                 & s \\ 
$r$              & Standstill distance   & 0      & --                 & m \\ 
\bottomrule
\end{tabular}  \vspace{-2mm}
\end{table}

%%%%  CONTROLLER REALIZATIONS %%%%%
We consider six different realizations, denoted by $F^l,\,l\in\{0,\ldots,5\}$, where $F^0$ corresponds to the base controller. The optimization problem is solved for a range of operating points $v_\text{r} \in [0,100]$~km/h. Although the optimal cost increases with $v_\text{r}$, the optimizer $f_{2,3}^*$ remains unchanged. Consequently, all results in the remainder of this section are solved for $v_\text{r}=50$~km/h.

The resulting controller realization matrices are summarized in TABLE~\ref{tab:realizations}. Realization $F^1$ modifies all realization entries except for $f_{2,3}$, which, according to Section~\ref{sec:uncertainCLdyn}, should yield identical closed-loop behavior to the base realization $F^0$ in the presence of uncertainty. Realizations $F^3$, $F^4$, and $F^5$ are obtained by solving~\eqref{eq:OP_OptProblem} with different objective functions. Since~\eqref{eq:OP_OptProblem} jointly minimizes $\mathrm{trace}(C_z P C_z^\top)$ and $\gamma$, the optimization problem is also solved for each objective individually to isolate their respective effects. Finally, a deliberately suboptimal realization $F^2$ is included to verify whether degraded performance is observed.
\begin{table}[bt]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Controller Realizations for Case Study Results.}
\label{tab:realizations} \vspace{-2mm}
\begin{tabular}{llll}
\toprule
 & \textbf{Objective} & $\mathbf{F}$ \\ 
\midrule
$F_0$ & Base controller & $[0,\,0,\,0,\, 0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_1$ & Equal performance & $[-\tfrac{\tau_i}{h_i},\,-\tfrac{\tau_i}{h_i},\,0,\,-\tfrac{\tau_i}{h_i},\,-\tfrac{\tau_i}{h_i}]$ \\
$F_2$ & Poor performance & $[0,\,0,\,0.3,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_3$ & Minimal $\mathrm{trace}(C_z P C_z^\top)$ + $\gamma$ & $[0,\,0,\,0.14865,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_4$ & Minimal $\mathrm{trace}(C_z P C_z^\top)$ & $[0,\,0,\,0.15866,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_5$ & Minimal $\gamma$ & $[0,\,0,\,0.11662,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
\bottomrule
\end{tabular} \vspace{-5mm}
\end{table} 


%%%%  SIMULATION RESULTS %%%%%
\subsection{Simulation Results} \vspace{-1mm}
The controller realizations in TABLE~\ref{tab:realizations} are evaluated in a MATLAB simulation of a two-vehicle platoon, consisting of a leader ($i=1$) and a follower ($i=2$). Model mismatch is introduced in the follower vehicle by setting all parameters at their lower bounds (TABLE~\ref{tab:vehicle_params}), together with a constant wind velocity $v_\text{w} = 15$~km/h. The leader tracks a reference velocity $v_\text{r}=15$~km/h and applies the following step input:
\begin{align} \label{eq:stepSimluation}
    u_1(t) = 
    \begin{cases}
        1 \quad & 10 \leq t\leq 11,\\
        -1 \quad & 21 \leq t\leq 22,\\
        0 \quad & \text{otherwise}.
        \end{cases}
\end{align}
The resulting follower velocity and spacing error are shown in Fig.~\ref{fig:sim_result} for each realization $F^l$, $l\!\in\!\!\{1,\ldots,5\}$. For reference, the nominal response (i.e., $\Delta = 0$) is included and is indicated by the solid black line.

To quantify the deviation between the uncertain and nominal closed-loop behavior, the root-mean-square error (RMSE) between $\zeta^0$ and $\zeta$ is reported in TABLE~\ref{tab:RMS_results}. Although the visual differences in Fig.~\ref{fig:sim_result} are subtle, the RMS values clearly demonstrate the superior performance of realization $F^5$. In contrast, the anticipated benefits of realization $F^4$ are not observed. While the objective $\mathrm{trace}(C_z P C_z^\top)$ targets transient deviations between $\zeta^0$ and $\zeta^e$, these effects are negligible in the present scenario. As a result, minimizing $\gamma$ dominates the performance, rendering $\mathrm{trace}(C_z P C_z^\top)$ ineffective as an objective in this case. The degraded performance of the suboptimal realization $F^2$ is clearly visible, while $F^1$ reproduces the behavior of the base controller $F^0$, as expected.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.96\linewidth]{00_Figures/velocity_and_error.eps} \vspace{-3mm}
    \caption{Time-domain simulation of a two-vehicle CACC platoon with parameters from TABLE~\ref{tab:vehicle_params} subject to parameter mismatch (uncertainties at lower bounds, positive wind velocity). Follower velocity $v_2$ and spacing error $e_2$ are shown for the controller realizations in TABLE~\ref{tab:realizations}.}
    \label{fig:sim_result} \vspace{-2mm}
\end{figure}

\begin{table}[bt]
\centering
\caption{Comparison of Velocity RMSE and Spacing RMSE}
\label{tab:RMS_results} \vspace{-2mm}
\begin{tabular}{lll}
\toprule
\textbf{Realization} & \textbf{Velocity RMSE} & \textbf{Spacing RMSE} \\
\midrule
$F^0$  & $0.0238\, (-)$ & $0.1554\, (-\%)$ \\
$F^1$   & $0.0238\, (-0\%)$ & $0.1554\, (-0\%)$ \\
$F^2$   & $0.0318\, (+34\%)$ & $0.2082\, (+33\%)$ \\
$F^3$   & $0.0186\, (-23\%)$ & $0.1550\, (-0.3\%)$ \\
$F^4$   & $0.0191\, (-20\%)$ & $0.1571\, (+1\%)$ \\
$F^5$   & $0.0179\, (-25\%)$ & $0.1498\, (-4\%)$ \\
\bottomrule
\end{tabular}  \vspace{-7mm}
\end{table}

%%%%  EXPERIMENTAL RESULTS %%%%%
\subsection{Experimental Results}  \vspace{-1mm}
The proposed controller realizations in TABLE~\ref{tab:realizations} are validated experimentally on the Renault Twizy test platform in Fig.~\ref{fig:twizyActionPic}, an electric vehicle equipped with a real-time computer for autonomous operation. Details on the vehicle hardware and software are provided in~\cite{de_haan_cooperative_2025}. The vehicle parameters and estimated uncertainty are listed in TABLE~\ref{tab:vehicle_params}.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.96\linewidth]{00_Figures/twizy_ITSC2.jpg} \vspace{-2mm}
    \caption{Renault Twizy experimental vehicle, details are provided in~\cite{de_haan_cooperative_2025}.}
    \label{fig:twizyActionPic}
    \vspace{-5mm}
\end{figure}
To complement the simulation study, an equivalent platooning scenario is implemented experimentally. A virtual leader is simulated on the follower vehicle’s real-time computer to enforce nominal leader dynamics. The virtual leader evolves according to the desired dynamics~\eqref{eq:desiredModel}, with $\tau_{i-1}=0.12$~s, tracks a reference velocity of $v_\text{r}=15$~km/h, and applies the step input defined in~\eqref{eq:stepSimluation}. Inter-vehicle distance is obtained by integrating the relative velocity. Experimental results are shown in Fig.~\ref{fig:step_twizy}. Transients at the start and end of the trajectory arise from cornering maneuvers required due to spatial constraints.

Overall, the experimental results align with the simulation study. In particular, the equivalence between realizations $F^0$ and $F^1$ is confirmed, as both yield nearly identical responses. The degraded performance of the suboptimal realization $F^2$ is clearly observable. Differences between realizations $F^3$, $F^4$, and $F^5$ are more subtle; nevertheless, realization $F^5$ exhibits the best overall performance, characterized by the smallest steady-state velocity error.

A subsequent experiment at $v_\text{r}=50$~km/h is performed, where $F^1$ and $F^2$ were omitted due to the established equivalence of $F^1$ with $F^0$ and the poor performance of $F^2$. The results in Fig.~\ref{fig:step_twizy_50} indicate that the vehicle is less affected by the model uncertainty at higher velocities, yielding similar responses across all tested realizations. This suggests that the nominal parameters align more closely with the true dynamics at this reference velocity, thereby reducing the model mismatch. Given that the parameter identification in Table~\ref{tab:vehicle_params} was obtained experimentally, the resulting nominal model is likely biased toward the higher-velocity data sets used during identification, potentially failing to represent low speeds sufficiently. The fact that all realizations yield similar responses in this test is not a limitation of the proposed method, but rather a positive. Since the system identification is velocity-dependent, it inherently introduces model mismatch across different velocities. The optimized PEC realizations provide the necessary robustness to compensate for this mismatch where it occurs (e.g., at low speeds), while exhibiting nominal behavior when the nominal parameters align with the true parameters.

Furthermore, although the overall conclusion remains the same, the experimental responses exhibit noticeably larger deviations from the leader than observed in the simulation. This discrepancy is likely due to unmodeled actuation delay. Including such delays in the simulation produces responses that better match the experimental data, as shown in Fig.~\ref{fig:act_delay}. Simulations indicate that actuation delay can reduce the benefits of optimized controller realizations relative to the base controller. Explicitly accounting for actuation delay in the PEC realizations, e.g., via a Padé approximation as in~\cite{de_haan_cooperative_2025}, may enable further performance improvements.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.96\linewidth]{00_Figures/step_twizy.eps} \vspace{-2mm}
    \caption{Experimental response of a Renault Twizy characterized by the parameters in TABLE~\ref{tab:vehicle_params}, tracking a virtual leader at 15 km/h. Follower velocity $v_2$ is shown for the realizations in TABLE~\ref{tab:realizations}.}
    \label{fig:step_twizy} \vspace{-2mm}
\end{figure}
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.96\linewidth]{00_Figures/step_twizy_50.eps} \vspace{-2mm}
    \caption{Experimental response of a Renault Twizy characterized by the parameters in TABLE~\ref{tab:vehicle_params}, tracking a virtual leader at 50 km/h. Follower velocity $v_2$ is shown for the realizations in TABLE~\ref{tab:realizations}. }
    \label{fig:step_twizy_50} \vspace{-2mm}
\end{figure}
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.96\linewidth]{00_Figures/act_delay.eps} \vspace{-2mm}
    \caption{Time-domain simulation of a two-vehicle CACC platoon with parameters from TABLE~\ref{tab:vehicle_params} subject to parameter mismatch (uncertainties at lower bounds, positive wind velocity) and $0.2$ s actuation delay. Follower velocity $v_2$ is shown for the controller realizations in TABLE~\ref{tab:realizations}.}
    \label{fig:act_delay} \vspace{-5mm}
\end{figure}




==> 6.Results_V2.tex <==
\section{Case Study Results} \label{sec:Results} \vspace{-2mm}

This section presents the design of the optimal PEC realization obtained by solving~\eqref{eq:OP_OptProblem}, followed by an evaluation on both MATLAB simulations and experiments on a Renault Twizy test platform. For both scenarios, we consider a two-vehicle platoon, with leader $i=1$ and follower $i=2$; in the experimental setup, the Renault Twizy tracks a virtual leader. The vehicle parameters and the associated parametric uncertainties (considered only for the follower vehicle) are summarized in Table~\ref{tab:vehicle_params}. The problem is solved in MATLAB~2025b using YALMIP~\cite{lofberg_yalmip_2004}, with solver MOSEK~\cite{mosek_aps_mosek_2024}.
\begin{table}[bt]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{Vehicle Parameters and estimated uncertainties.}
\label{tab:vehicle_params} \vspace{-3mm}
\begin{tabular}{llccc}
\toprule
\textbf{Sym.} & \textbf{Parameter} & \textbf{Nominal} & \textbf{Range ($\Delta$)} & \textbf{Unit} \\ 
\midrule
$m$              & Vehicle Mass          & 731      & $[716, 746]$       & kg \\
$m_{\text{eff}}$ & Effective Mass        & 778      & $[763, 793]$       & kg \\
$f_v$            & Viscous Friction      & 5.55     & $[5.5, 5.6]$       & Ns/m \\
$f_r$            & Rolling Res. Coeff.   & 0.0262   & $[0.0262, 0.0262]$ & -- \\
$C_d$            & Aero. Drag Factor     & 0.392    & $[0.3528, 0.4312]$ & kg/m \\
$\tau$           & Time Constant         & 0.12     & $[0.11, 0.13]$     & s \\
$\alpha$         & Road Slope            & 0        & $[0, 0]$           & rad \\
$v_{\text{w}}$   & Wind Velocity         & 0        & $[-5, 5]$          & m/s \\
$(k_p,k_d)$      & Prop./Deriv. gain     & (0.2,0.7)& --                 & (1/s$^2$,1/s) \\ 
$h$              & Headway time          & 0.2      & --                 & s \\ 
%$r$              & Standstill distance   & 0        & --                 & m \\ 
\bottomrule
\end{tabular}  %\vspace{-7mm}
\end{table}

Six different PEC realizations, denoted by $F^l,\,l\in\{0,\ldots,5\}$, are evaluated. $F^0$ is the base controller. $F^1$ modifies all entries except for $f_{2,3}$, which, as discussed in Section~\ref{sec:uncertainCLdyn}, theoretically yields identical closed-loop behavior to $F^0$ under uncertainty. $F^2$ is a deliberately suboptimal realization to verify whether degraded performance is observed. Furthermore, realizations $F^3$, $F^4$, and $F^5$ are obtained by solving~\eqref{eq:OP_OptProblem} with different objective functions; while~\eqref{eq:OP_OptProblem} jointly minimizes $\mathrm{trace}(C_z P C_z^\top)$ and $\gamma$, the optimization problem is solved for each objective individually to isolate their respective effects. The optimization problem is solved for a range of operating points $v_\text{r} \in [0,100]$~km/h. Although the optimal cost increases with $v_\text{r}$, the optimizer $f_{2,3}^*$ appeared invariant. Consequently, all subsequent results are obtained using $v_\text{r} = 15 $~km/h. The resulting PEC matrices are summarized in TABLE~\ref{tab:realizations}. 
\begin{table}[bt]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{PEC Realizations for Case Study Results.}
\label{tab:realizations} \vspace{-3mm}
\begin{tabular}{llll}
\toprule
 & \textbf{Objective} & $\mathbf{F}$ \\ 
\midrule
$F_0$ & Base controller & $[0,\,0,\,0,\, 0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_1$ & Equal performance & $[-\tfrac{\tau_i}{h_i},\,-\tfrac{\tau_i}{h_i},\,0,\,-\tfrac{\tau_i}{h_i},\,-\tfrac{\tau_i}{h_i}]$ \\
$F_2$ & Poor performance & $[0,\,0,\,0.3,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_3$ & Minimal $\mathrm{trace}(C_z P C_z^\top)$ + $\gamma$ & $[0,\,0,\,0.14865,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_4$ & Minimal $\mathrm{trace}(C_z P C_z^\top)$ & $[0,\,0,\,0.15866,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
$F_5$ & Minimal $\gamma$ & $[0,\,0,\,0.11662,\,0,\,-\tfrac{\tau_i}{h_i}]$ \\
\bottomrule
\end{tabular} %\vspace{-3mm}
\end{table} 

%%%%  SIMULATION RESULTS %%%%%
\subsection{Simulation Results} \vspace{-1mm}
In the simulation, we evaluate the nonlinear model~\eqref{eq:CL_PEC_uncertain} with a constant wind speed $v_\text{w} = 15$~km/h, and set the follower vehicle parameters at their lower bounds (TABLE~\ref{tab:vehicle_params}) to introduce a model mismatch. The leader tracks a reference velocity $v_\text{r}=15$~km/h and applies the step input $u_1(t) = 1$ for $t \in [10, 11]$, $-1$ for $t \in [21, 22]$, and $0$ otherwise.

The resulting follower velocity and spacing error for each realization $F^l, \, l \in \{1, \dots, 5\}$ are illustrated in Fig.~\ref{fig:sim_result}, with the nominal response ($\Delta = 0$) provided as a baseline (solid black line). To quantify the deviation between the uncertain and nominal closed-loop behavior, the root-mean-square error (RMSE) between $\zeta^0$ and $\zeta$ is reported in Table~\ref{tab:RMS_results}. Although the visual differences in Fig.~\ref{fig:sim_result} are subtle, Table~\ref{tab:RMS_results} highlights the superior performance of realization $F^5$. Interestingly, the anticipated benefits of $F^4$ are not observed in this scenario. While the objective $\mathrm{trace}(C_z P C_z^\top)$ is designed to mitigate transient deviations in the error state $\zeta^e$, these effects appear to be negligible here. Consequently, the performance is dominated by the minimization of $\gamma$, rendering the trace objective ineffective in this specific case. Finally, the suboptimal realization $F^2$ exhibits degraded performance, while $F^1$ successfully reproduces the baseline behavior of $F^0$, confirming the theoretical expectations.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.9\linewidth]{00_Figures/ITSC_simulation_revision.eps} \vspace{-3mm}
    \caption{Follower velocity $v_2$ and spacing error $e_2$ for the PEC realizations $F^l, l\in\{1,...,5\}$, in TABLE~\ref{tab:realizations}.}
    \label{fig:sim_result} %\vspace{-2mm}
\end{figure}
\begin{table}[bt]
\centering
\caption{Comparison of Velocity RMSE and Spacing RMSE}
\label{tab:RMS_results} \vspace{-3mm}
\begin{tabular}{lll}
\toprule
\textbf{Realization} & \textbf{Velocity RMSE} & \textbf{Spacing RMSE} \\
\midrule
$F^0$  & $0.0238\, (-)$ & $0.1554\, (-\%)$ \\
$F^1$   & $0.0238\, (-0\%)$ & $0.1554\, (-0\%)$ \\
$F^2$   & $0.0318\, (+34\%)$ & $0.2082\, (+33\%)$ \\
$F^3$   & $0.0186\, (-23\%)$ & $0.1550\, (-0.3\%)$ \\
$F^4$   & $0.0191\, (-20\%)$ & $0.1571\, (+1\%)$ \\
$F^5$   & $0.0179\, (-25\%)$ & $0.1498\, (-4\%)$ \\
\bottomrule
\end{tabular}  %\vspace{-7mm}
\end{table}

%%%%  EXPERIMENTAL RESULTS %%%%%
\subsection{Experimental Results}  \vspace{-1mm}
To complement the simulation study, the platooning scenario is validated experimentally using the Renault Twizy in Fig.~\ref{fig:twizyActionPic}, with details on the vehicle in~\cite{de_haan_cooperative_2025}. A virtual leader is implemented on the follower vehicle's real-time computer to enforce the desired nominal dynamics \eqref{eq:desiredModel}. The leader tracks a reference velocity $v_\text{r} = 15$~km/h and applies the same input $u_1$ as in the simulation, while the inter-vehicle distance is obtained by integrating the relative velocity. The experimental results are shown in Fig.~\ref{fig:step_twizy}. The transients observed at the start and end of the trajectory are artifacts of the cornering maneuvers required due to spatial constraints.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.7\linewidth]{00_Figures/twizy_ITSC2.jpg} \vspace{-3mm}
    \caption{Renault Twizy experimental vehicle, details in~\cite{de_haan_cooperative_2025}.}
    \label{fig:twizyActionPic}
    %\vspace{-5mm}
\end{figure}

Overall, the experimental data align with the simulation results. Specifically, the equivalence between realizations $F^0$ and $F^1$ is confirmed, as both yield nearly identical velocity profiles. The performance degradation associated with the suboptimal realization $F^2$ remains clearly observable under real-world conditions. While the performance differences between $F^3$, $F^4$, and $F^5$ are more subtle, realization $F^5$ consistently exhibits the best response, characterized by the smallest steady-state velocity error.
\begin{figure}[bt]
    \centering
    \includegraphics[width=0.9\linewidth]{00_Figures/Experiment_revision_V2.eps} \vspace{-2mm}
    \caption{Measured follower velocity $v_2$ for the PEC realizations $F^l, l\in\{1,...,5\}$, tracking a virtual leader at 15 km/h.}
    \label{fig:step_twizy} %\vspace{-2mm}
\end{figure}




\begin{comment}
    \begin{small} \begin{align} \label{eq:stepSimluation}
  u_1(t) = 
    \begin{cases}
        1 \quad & 10 \leq t\leq 11,\\
        -1 \quad & 21 \leq t\leq 22,\\
        0 \quad & \text{otherwise}.
        \end{cases} 
\end{align}\end{small}

\begin{figure}[bt]
    \centering
    \includegraphics[width=0.8\linewidth]{00_Figures/step_twizy.eps} \vspace{-2mm}
    \caption{Measured follower velocity $v_2$ for the PEC realizations $F^l, l\in\{1,...,5\}$, tracking a virtual leader at 15 km/h.}
    \label{fig:step_twizy} %\vspace{-2mm}
\end{figure}
\end{comment}
    


==> BennSpacing.tex <==
%%%%%%%%%%%%%%% BENN %%%%%%%%%%%%%%%%%%%%%
%% Float Caption Compression
\setlength{\abovecaptionskip}{0.4\baselineskip}
\setlength{\belowcaptionskip}{0.25\baselineskip}

%% Float <-> text compression
\setlength{\textfloatsep}{1ex}   % Distance between float and text
\setlength{\floatsep}{1ex}     % Distance between floats
\setlength{\dblfloatsep}{1ex}      % Distance between two column floats
\setlength{\dbltextfloatsep}{1ex}  % Distance between two column floats and text

%% Footnote compression
%\setlength{\skip\footins}{1ex}

%% Header Spacing
\makeatletter
\renewcommand{\section}{\@startsection{section}{1}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
	{0.7ex plus 1ex minus 0ex}{\normalfont\normalsize\centering\scshape}}%
\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
	{0.7ex plus 1ex minus 0ex}{\normalfont\normalsize\itshape}}%
\makeatother


%% Equation compression
\expandafter\def\expandafter\normalsize\expandafter{%
\normalsize
\setlength\abovedisplayskip{5pt}
\setlength\belowdisplayskip{5pt}
\setlength\abovedisplayshortskip{5pt}
\setlength\belowdisplayshortskip{5pt}
}

\widowpenalty10000
\clubpenalty10000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
